Non-convex Bayesian Learning via Stochastic Gradient Markov Chain Monte Carlo

The rise of artificial intelligence (AI) hinges on the efficient training of modern deep neural networks (DNNs) for non-convex optimization and uncertainty quantification, which boils down to a non-convex Bayesian learning problem. A standard tool to handle the problem is Langevin Monte Carlo, which proposes to approximate the posterior distribution with theoretical guarantees. In this thesis, we start with the replica exchange Langevin Monte Carlo (also known as parallel tempering), which proposes appropriate swaps between exploration and exploitation to achieve accelerations. However, the na\"ive extension of swaps to big data problems leads to a large bias, and bias-corrected swaps are required. Such a mechanism leads to few effective swaps and insignificant accelerations. To alleviate this issue, we first propose a control variates method to reduce the variance of noisy energy estimators and show a potential to accelerate the exponential convergence. We also present the population-chain replica exchange based on non-reversibility and obtain an optimal round-trip rate for deep learning. In the second part of the thesis, we study scalable dynamic importance sampling algorithms based on stochastic approximation. Traditional dynamic importance sampling algorithms have achieved success, however, the lack of scalability has greatly limited their extensions to big data. To handle this scalability issue, we resolve the vanishing gradient problem and propose two dynamic importance sampling algorithms. Theoretically, we establish the stability condition for the underlying ordinary differential equation (ODE) system and guarantee the asymptotic convergence of the latent variable to the desired fixed point. Interestingly, such a result still holds given non-convex energy landscapes.

==> others/ap-about-appendices.tex <==
\ProvidesFile{ap-about-appendices.tex}[2021-08-23 about the appendicies appendix]

\begin{VerbatimOut}{z.out}
\chapter{ABOUT THE APPENDICES}

% Use single spacing in the appendices from now on to save space.
\ZZbaselinestretch{1}

\textcolor{red}{%
  \textbf{%
    These appendices are single-spaced to save space.
    Your thesis should use the default~1.5 line spacing.%
  }%
}

There are two groups of appendices.
The first group are general appendices;
the second group are domain-specific appendices.

These appendices are a series of examples.
They are a work in progress.

Each example consists of some \LaTeX\ output
followed by the corresponding input lines.
Some \LaTeX\ input lines only define things
and don't produce any output.
Each chunk in the input file begins with
\verb+\begin{VerbatimOut}{z.out}+
then has the \LaTeX\ input for the example,
% Don't literally end VerbatimOut on next line.
and ends with {\tt \char'134 end\char'173 VerbatimOut\char'175},
followed by a blank line,
followed by a line that begins with
\verb+\My+.

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

  
\section{Paragraphs}

This is the first paragraph.
Paragraphs are separated by blank lines.

This is the second paragraph.


\section{Section Heading}

This is a sentence.
This is a sentence.
This is a sentence.
This is a sentence.
This is a sentence.


\subsection{Subsection heading}

This is a sentence.
This is a sentence.
This is a sentence.
This is a sentence.
This is a sentence.


\subsubsection{Subsubsection heading}

This is a sentence.
This is a sentence.
This is a sentence.
This is a sentence.
This is a sentence.
\end{VerbatimOut}

\MyIO



\begin{VerbatimOut}{z.out}


\section{Text math}

If items in a list are narrow like these Greek characters,\\
    \I2 \verb+$\alpha$, $\beta$, and $\gamma$+\\
I'd input the line like this\\
    \I2 \verb+$\alpha$,~$\beta$, and~$\gamma$+\\
where the \verb+~+ is a tie
that ties together what's before and after it on the same line of the output
\cite[page~92]{knuth2012}.

This text is the correct length to show what happens with and without ties:
$\alpha$,
$\beta$,
and $\gamma$.
See how the line gets split
and the~$\gamma$ is at the beginning of the line?

This text is the correct length to show what happens with and without ties:
$\alpha$,~$\beta$,
and~$\gamma$.
See how the line gets compressed a little bit so the~$\gamma$
is not at the beginning of the line?
\end{VerbatimOut}

\MyIO


==> others/ap-astronomy.tex <==
\ProvidesFile{ap-astronomy.tex}[2021-08-23 astronomy appendix]

\begin{VerbatimOut}{z.out}
\chapter{ASTRONOMY}
\ix{astronomy//Astronomy appendix}

\ix{astronomy}  

\end{VerbatimOut}

\MyIO


==> others/ap-biology.tex <==
\ProvidesFile{ap-biology.tex}[2021-08-23 biology appendix]

\begin{VerbatimOut}{z.out}
\chapter{BIOLOGY}

\ix{Biology chapter}
\end{VerbatimOut}

\MyIO


==> others/ap-bugs.tex <==
\ProvidesFile{ap-bugs}[2021-08-23 bugs appendix]

\newcommand{\bug}{\vspace{6pt}}  
\newcommand{\checkedok}[1]{{\bfseries Checked ok on #1.}}
\newcommand{\waitingon}[1]{{\bfseries Waiting on #1.}}

\chapter{BUGS}

See ap-bugs.tex file for \LaTeX\ input.


\section{These problems need to be fixed}

% I need to fix the following things in \PurdueThesis.
% They are listed in decreasing order in priority.

\bug
Allow manual line break in \verb+\title+.
{\small (Mark Senn <mark@purdue.edu>.)}

\bug
Allow comma in \verb+\title+.
{\small (Mark Senn <mark@purdue.edu>).}

\bug
Table of Contents uses double-spaced instead of 1\sfrac12 spacing.
Tighten up section and less significant heading spacing?
{\small (Anita Adams Sale <aasale@iupui.edu>, 2021-03-17, 11:16.)}
 
\bug
List of Figures indented $\approx$\sfrac14 inch
more than List of Tables.
{\small (Anita Adams Sale <aasale@iupui.edu>, 2021-03-17, 11:16.)}

\bug
Left reference section margin is ok if a person has 10--99 references.
Figure out how to adjusting margin for 1--9 or over 99 references.
{\small (Mark Senn <mark@purdue.edu>.)}

\bug
Change citation, e.g., ``[6], [71]'' to ``[6,71]''.
{\small (Mark Senn <mark@purdue.edu>, 2021-04-07, 11:55.)}

\bug
Change citation, e.g., ``[6], [7], [8]'' to ``[6-8]''.
{\small (Mark Senn <mark@purdue.edu>, 2021-04-07, 11:55.)}

\bug
APA reference style indents references too far on left.
{\small (Mark Senn <mark@purdue.edu>, 2021-04-08, 21:42.)}

\bug
Use ``Last Accessed: dd/mm/yy.'' urldate in bibliography.
{\small (Priyank Kalgaonkar <pkalgaon@iupui.edu>, 2021-04-06, 15:58.)}

\bug
Use ``Last Accessed: yyyy-mm-dd.'' urldate in bibliography.
{\small (Mark Senn <mark@purdue.edu>, 2021-04-19, 17:05.)}

\bug
Check that \verb+@{}+ is before the left column
and after the right column in all tables.
{\small (Mark Senn <mark@purdue.edu>, 2021-04-19, 21:32.)}

\bug  
Add DTECH degree.


\section{These issues have been reported}

\bug
Bibliography change.
Change,
for example,
``Acoustical Science and Technology, vol.~23, no.~1''
to
``Acoustical Science and Technology {\bfseries 23\/} ({\bfseries 1\/})''.
{\small (Daniel Joesph Carr <djcarr@purdue.edu>, 2021-06-16, 09:33.)}

\bug
Bibliography change.
Change,
for example,
``M.~Abramowitz and I.A.~Stegun, Eds.,''
to
``M.~Abramowitz and I.A.~Stegun, editors,''
{\small (Daniel Joesph Carr <djcarr@purdue.edu>, 2021-06-16, 09:33.)}

\bug
Section headings containing a SmallCaps font do not work.
{\small (Javad (Nima) Darivandpour" <jdarivan@purdue.edu>, 2021-06-29, 10:25.}
See \ref{section-headings-with-smallcaps-font}

\section{These problems are waiting on a reply}

\verb+linktoc = section+ does not work with captions with \verb+\frac+.
{\small
  (Mark Senn <mark@purdue.edu>, 2021-05-27, 13:09.
  In the short-term check with Ashlee Messersmith <amiley@purdue.edu>
  if \verb+linktoc = page+ can be used.
  If that's ok make the change
  and look into changing captions from my code
  to \LaTeX's code.)%
}
\waitingon{Ashlee}


\section{These problems have been fixed}

Non-nested description environments have bold items.
Nested description environments have non-bold items.
How come?
Are the indentations correct?
{\small (Mark Senn <mark@purdue.edu>, 2021-04-09, 16:49.)}
\checkedok{2021-05-31}



==> others/ap-chapter-appendices.tex <==
\ProvidesFile{ap-chapter-appendices.tex}[2021-08-23 chapter appendices appendix]

\begin{VerbatimOut}{z.out}
\chapter{CHAPTER APPENDICES}

Using \verb+\chapterappendix+ or \verb+\chapterappendices+
in the first chapter will number sections, for example,
1.1, 1.2, 1.A.

Using \verb+\chapterappendix+ or \verb+\chapterappendices+
in the first appendix will number sections, for example,
A.1, A.2, A.A.

Only use \verb+\chapterappendix+ or \verb+\chapterappendices+
in chapters.
Using them in appendices is too confusing.

\section{This is a section headings}

This is a paragraph.

Use \verb+\chapterappendix+ or \verb+chapterappendices+
to make sections until the end of the next chapter
be appendices.

\chapterappendix

\section{This is a chapter appendix}

This is a paragraph.
\end{VerbatimOut}

\MyIO


==> others/ap-chapter-references.tex <==
\ProvidesFile{ap-chapter-references.tex}[2021-08-23 chapter references appendix]

\begin{VerbatimOut}{z.out}
\begin{refsection}
\chapter{CHAPTER REFERENCES}

This is a paragraph.

\section{This is a section heading}

This is a paragraph.

\verb+\cite{reid2013}+ gives \cite{reid2013}.
\verb+\cite{test-long-title}+ gives \cite{test-long-title}.
\verb+\cite{sexon2012}+ gives \cite{sexon2012}.
\verb+\cite{test-long-titleb}+ gives \cite{test-long-titleb}.

\PrintChapterBibliography
\end{refsection}
\end{VerbatimOut}

\MyIO


==> others/ap-check-margins.tex <==
\ProvidesFile{ap-check-margins.tex}[2021-08-23 check margins appendix]

\begin{VerbatimOut}{z.out}
\chapter{CHECK MARGINS}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\MyRepeat{This is a sentence. }{300}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
{
  \tiny
  \MyRepeat{This is a sentence. }{600}
}
\end{VerbatimOut}


==> others/ap-chemistry.tex <==
\ProvidesFile{ap-chemistry.tex}[2021-08-23 chemistry appendix]

\begin{VerbatimOut}{z.out}
\chapter{CHEMISTRY}
\label{ch:chemistry}

\ix{chemistry}
\ix{Chemistry appendix}

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Chemical Diagrams}

The chemplants package \cite{feffin2019}
extends the
\href{http://ctan.math.washington.edu/tex-archive/graphics/pgf/base/doc/pgfmanual.pdf}{\TikZLogo} package
to draw chemical process units.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Chemical Equations}

The mhchem Bundle \cite{hensel2018}
contains mhchem v4.08 (chemical equations),
hpstatement v1.02 (official hazard and precautionary statements),
and rsphrase v3.11 (official rist and safety phrases).
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Defined in thesis.tex: \nitrate.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% See page 1 of
%     https://www.thoughtco.com/what-is-a-chemical-equation-604026
\ce{CH4 + 2O2 -> CO2 + 2H2O}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% See page 1 of
%     https://www.thoughtco.com/what-is-a-chemical-equation-604026
\ce{2H2(g) + O2(g) -> 2H2O(l)}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% See page 1 of
% https://www.thoughtco.com/definition-of-ionic-equation-605262
\ce{Ag+(aq) + NO3-(aq) + Na+(aq) + Cl-(aq) -> AgCl(s) + Na+(aq) + NO3-(aq)}
is an ionic equation of the chemical reaction:
\ce{AgNO3(aq) + NaCl(aq) -> AgCl(s) + NaNO3(aq)}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% See page 1 of
%     https://www.thoughtco.com/definition-of-balanced-equation-and-examples-604380
\ce{Fe2O3 + C -> Fe + CO2}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% From page 1 of
%     https://www.thoughtco.com/definition-of-molecular-equation-605366

For example, in the reaction between sodium chloride
(\ce{NaCl})
and silver nitrate
(\ce{AgNO3}),
the molecular reaction is:

\ce{NaCl(aq) + AgNO3 -> NaNO3(aq) + AgCl(s)}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The complete ionic equation is:

\ce{Na+(aq) + Cl-(aq) + Ag+(aq) + NO3-(aq) -> AgCl(s) + Na+(aq) + NO3-(aq)}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Ruben Meerman \cite[starting at 5:25]{meerman} claims this equation
\begin{center}
  \ce{C55H104O6 + 78O2 -> 55CO2 + 52H2O + energy}\endgraf
\end{center}
describes weight loss.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

And with better annotation:

\begin{center}
  \newcommand{\vph}{{\vphantom{\large Ag}}}
  \ce{
    $\underset{\text{\vph \footnotesize human fat}}{\ce{C55H104O6}}$
    +
    $\underset{\text{\vph \footnotesize oxygen}}{\ce{78O2}}$
    ->
    $\underset{\text{\vph \footnotesize carbon dioxide}}{\ce{55CO2}}$
    +
    $\underset{\text{\vph \footnotesize water}}{\ce{52H2O}}$
    +
    $\underset{\text{\vph \footnotesize body heat, moving, thinking, growing}}{\text{energy}}$
  }
\end{center}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

And with still better annotation:

\begin{center}
  \newcommand{\Fs}{\scriptsize}
  \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
    &                                                       %  1. C55H10406
      &                                                     %  2. +
      &                                                     %  3. 78O2
      &                                                     %  4. ->
      &                                                     %  5. 55CO2
      &                                                     %  6. +
      &                                                     %  7. 52H2O
      &                                                     %  8. +
      \Fs calories\\                                        %  9. energy
    %
    \Fs kg&                                                 %  1.
      &                                                     %  2.
      \Fs kg&                                               %  3.
      &                                                     %  4.
      \Fs kg&                                               %  5.
      &                                                     %  6.
      \Fs kg&                                               %  7.
      &                                                     %  8.
      \Fs kJ\\                                              %  9.
    %
    \noalign{\vspace{3pt}}
    %
    \ce{C55H104O6}                                          %  1.
      & \ce{+}                                              %  2.
      & \ce{78O2}                                           %  3.
      & \ce{->}                                             %  4.
      & \ce{55CO2}                                          %  5.
      & \ce{+}                                              %  6.
      & \ce{52H2O}                                          %  7.
      & \ce{+}                                              %  8.
      & energy\\                                            %  9.
    %
    \Fs human fat&                                          %  1.
      &                                                     %  2.
      \Fs oxygen&                                           %  3.
      &                                                     %  4.
      \Fs carbon dioxide&                                   %  5.
      &                                                     %  6.
      \Fs water&                                            %  7.
      &                                                     %  8.
      \Fs body heat, moving, thinking, growing\\            %  9.
  \end{tabular}
\end{center}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Chemical Figures}

Below is an example of how to use the chemfig package \cite{tellechea2021}.

% Chicago Manual of Style Online, 17 edition, section 9.61 states
% that 72--73, not 72--3, should be used.
Here is the chemical figure
for Penicillin \cite[pages~72--73]{tellechea2021}:\\

\chemfig{
  [:-90]HN(-[::-45](-[::-45]R)=[::+45]O)>[::+45]*4(-(=O)-N*5(-(<:(=[::-60]O)
  -[::+60]OH)-(<[::+0])(<:[::-108])-S>)--)
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\newpage
\section{Chemical Schemes}

Below are some examples of how to do schemes.

\begin{scheme}[ht]
  \caption{This is the first scheme caption.}
  \vspace*{6pt}
  \begin{center}
    This is the first scheme.
  \end{center}
\end{scheme}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\begin{scheme}[ht]
  \caption{This is the second scheme caption.}
  \vspace*{6pt}
  \begin{center}
    % Next line was added to make scheme a little smaller.
    \scriptsize\setchemfig{bond offset=1pt,atom sep=3em,compound sep=6em}
    \schemestart
      \chemfig{-[:30](-[2])-[:-30]OH}
      \arrow
      \chemfig{-[:30](-[2])=^[:-30]O}
    \schemestop
  \end{center}
\end{scheme}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\newpage
\begin{scheme}[ht]
  \caption{%
    The Fischer indole synthesis
    \cite[pages~74--75]{tellechea2021}.%
  }
  \vspace*{6pt}
  \begin{center}
    % Next line was added to make scheme a little smaller.
    \scriptsize\setchemfig{bond offset=1pt,atom sep=3em,compound sep=6em}
    \schemestart
      \chemfig{*6(=-*6(-\chembelow{N}{H}-NH_2)=-=-)}
      \+
      \chemfig{(=[:-150]O)(-[:-30]R_2)-[2]-[:150]R_1}
      \arrow(.mid east--.mid west){->[\chemfig{H^+}]}
      \chemfig{*6(-=*5(-\chembelow{N}{H}-(-R_2)=(-R_1)-)-=-=)}
    \schemestop
  \end{center}
\end{scheme}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\newpage
\begin{scheme}[ht]
  \caption{%
    The Cannizzaro reaction
    \cite[pages~77--78]{tellechea2021}.%
  }
  \vspace*{12pt}
  \begin{center}
    % Next line was added to make scheme a little smaller.
    \scriptsize\setchemfig{bond offset=1pt,atom sep=3em,compound sep=6em}
    \schemestart
      \chemfig{[:-30]*6(=-=(-@{atoc}C([6]=[@{db}]@{atoo1}O)-H)-=-)}
      \arrow(start.mid east--.mid west){->[\chemfig{@{atoo2}\chemabove{O}{\scriptstyle\ominus}}H]}
      \chemmove[-stealth,shorten >=2pt,dash pattern=on 1pt off 1pt,thin]{
        \draw[shorten <=8pt](atoo2) ..controls +(up:10mm) and +(up:10mm)..(atoc);
        \draw[shorten <=2pt](db) ..controls +(left:5mm) and +(west:5mm)..(atoo1);}
      \chemfig{[:-30]*6(=-=(-C([6]-[@{sb1}]@{atoo1}\chembelow{O}{\scriptstyle\ominus})
        ([2]-OH)-[@{sb2}]H)-=-)}
      \hspace{1cm}
      \chemfig{[:-30]*6((-@{atoc}C([6]=[@{db}]@{atoo2}O)-[2]H)-=-=-=)}
      \chemmove[-stealth,shorten <=2pt,shorten >=2pt,dash pattern=on 1pt off 1pt,thin]{
        \draw([yshift=-4pt]atoo1.270) ..controls +(0:5mm) and +(right:10mm)..(sb1);
        \draw(sb2) ..controls +(up:10mm) and +(north west:10mm)..(atoc);
        \draw(db) ..controls +(right:5mm) and +(east:5mm)..(atoo2);}
      \arrow(@start.base west--){0}[-75,2]
      {}
      \arrow
      \chemfig{[:-30]*6(=-=(-C([1]-@{atoo2}O-[@{sb}0]@{atoh}H)([6]=O))-=-)}
      \arrow{0}
      \chemfig{[:-30]*6((-C(-[5]H)(-[7]H)-[2]@{atoo1}\chemabove{O}{\scriptstyle\ominus})-=-=-=)}
      \chemmove[-stealth,shorten >=2pt,dash pattern=on 1pt off 1pt,thin]{
        \draw[shorten <=7pt](atoo1.90) ..controls +(+90:8mm) and +(up:10mm)..(atoh);
        \draw[shorten <=2pt](sb) ..controls +(up:5mm) and +(up:5mm)..(atoo2);}
    \schemestop
  \end{center}
\end{scheme}
\end{VerbatimOut}

\MyIO


%\begin{scheme}[ht]
%  \caption{This is the third scheme caption.}
%  \vspace*{6pt}
%  \begin{center}
%    \schemestart
%      \chemfig{*6(=-=(-(=[2]O)-[%-60]O-[0]O-[%30](=[2]O)-[%-60]*6(=-=-=-))=-)}
%      \arrow{->[$\Delta$]}
%      2 \chemfig{*6(=-=(-(=[2]O)-[%-60]{0.,0})-=-)}
%      \arrow
%      2 \chemfig{*6(=-=(-[,.15,,,draw-none]{0.,})-=-)}\+\ch{2 CO2 ^}
%    \schemestop
%  \end{center}
%\end{scheme}


==> others/ap-citations-references.tex <==
\ProvidesFile{ap-citations.tex}[2021-08-23 citations and references appendix]

\begin{VerbatimOut}{z.out}
\chapter{CITATIONS AND REFERENCES}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
This chapter contains information about citations
and references---how to cite a reference in the text
and the fine points of defining a bibliography
(also called ``References'')
entry.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\section{Citations}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
For \LaTeX\ answers I refer to
\cite{lamport1994}
and then to
\cite{goossens1994}
or
\cite{kopka1999}.
\cite{kopka1999}
is an update to \cite{kopka1995} (the 1995 edition).
\end{VerbatimOut}

\MyIO


Here is an example .bib file entry:

\begin{VerbatimOut}{z.out}
@misc{example2020,
  address   = {Imaginaryville, Indiana},
  author    = {Andrew Anteater and Bertha Bear and Charles Cheetah and Davida Deer and Ethan Eagle},
  date      = {2020-10-27},
  doi       = {00.0000/000-0-000-00000-0},
  editor    = {Mark Senn},
  edition   = {2},
  isbn      = {{000\FigureDash 0\FigureDash 000\FigureDash 00000\FigureDash 0}},
  publisher = {Bogus International Publishing Company},
  title     = {An Imaginary Document Not About {Mark Senn} or {NASA}},
  url       = {https://bogus.com/bogus.html},
  urldate   = {2020-10-27},
  version   = {1.0},
}
\end{VerbatimOut}

\MyIO


Here are some example BibLaTeX citations.
Depending on the style being used these will produce different results.

\mbox{}\\
\begin{tabular}{@{}ll@{}}
  \bf Input&                        \bf Output\\
  \verb+\cite{example2020}+&        \cite{example2020}\\
  \verb+\cite*{example2020}+&       \cite*{example2020}\\
  \verb+\citeauthor{example2020}+&  \citeauthor{example2020}\\
  \verb+\citeauthor*{example2020}+& \citeauthor*{example2020}\\
  \verb+\citedate{example2020}+&    \citedate{example2020}\\
  \verb+\citetitle{example2020}+&   \citetitle{example2020}\\
  \verb+\citetitle*{example2020}+&  \citetitle*{example2020}\\
  \verb+\citeurl{example2020}+&     \citeurl{example2020}\\
  \verb+\citeyear{example2020}+&    \citeyear{example2020}\\
  \verb+\parencite{example2020}+&   \parencite{example2020}\\
  \verb+\textcite{example2020}+&    \textcite{example2020}\\
\end{tabular}

\begin{VerbatimOut}{z.out}
\section{References}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
  Emily Spreen wrote that the following URLs are invisible in the PDF file.
  They worked fine for me on 2021-04-08.
  See \cite{hambleton}, \cite{gerstenmaier}, and \cite{gerstenmaier2} in the REFERENCES.

{\footnotesize
\begin{verbatim}
@misc{hambleton,
  key = {Deep Space Gateway},
  title = {{Deep Space Gateway to Open Opportunities for Distant Destinations}},
  note = {Editor: Kathryn Hambleton},
  year = {2018},
  month = {August 24,},
  howpublished = {\url{https://www.nasa.gov/feature/deep-space-gateway-to-open-...}},
  organization = {NASA},
}
\end{verbatim}
}

{\footnotesize
\begin{verbatim}
@misc{gerstenmaier,
  author = {William H. Gerstenmaier},
  title = {{Progress in Defining the Deep Space Gateway and Transport Plan}},
  month = {March},
  year = {2017},
  howpublished = {\url{https://www.nasa.gov/sites/default/files/atoms/files/...}},
  organization = {NASA},
}
\end{verbatim}
}

I suggest using the following
(added a `2' to the key so they'd have separate entries in the references.).
{\footnotesize
\begin{verbatim}
@misc{gerstenmaier2,
  author = {William H. Gerstenmaier},
  date = {2017-03},
  title = {{Progress in Defining the Deep Space Gateway and Transport Plan}},
  url = {https://www.nasa.gov/sites/default/files/atoms/files/nss_chart_v23.pdf},
  organization = {NASA},
}
\end{verbatim}
}
\end{VerbatimOut}



\MyIO


==> others/ap-colophon.tex <==
\ProvidesFile{ap-colophon.tex}[2021-08-23 colophon]

\begin{VerbatimOut}{z.out}
\chapter*{COLOPHON}
\label{ap:colophon}

\ix{colophon}

This is the colophon.

\end{VerbatimOut}

\MyIO


==> others/ap-common-mistakes.tex <==
\ProvidesFile{ap-common-mistakes.tex}[2021-08-23 common mistakes appendix]

\begin{VerbatimOut}{z.out}
\chapter{COMMON MISTAKES}

The following Headings, Mathematics, and Text
sections describe some common mistakes.


\section{Headings}

\ifthen{\equal{\bibprocessor}{biblatex}}
{\textcite[page~289]{farkas2011} }%
\ifthen{\equal{\bibprocessor}{bibtex}}
{\cite{farkas2011} }%
wrote

\begin{quotation}
  The practice of stacking headings
  is routinely condemned by style manuals
  and other authorities.
  Here is a typical statement,
  taken from Houghton Mifflin's guidelines for authors.
  \begin{quotation}
    Avoid ``stacking'' heads,
    or placing two levels
    of headings together without intervening text.
    A heading cannot substitute
    for the transitional
    or introductory paragraphs
    that guide the reader through a chapter.
    Remember too that a chapter opening looks better in type
    when one
    or more paragraphs
    of text precede the first heading.
  \end{quotation}
\end{quotation}
\end{VerbatimOut}

\MyIO

\begin{VerbatimOut}{z.out}


\section{Mathematics}

\subsection{Put a little extra horizontal space before dx.}
\end{VerbatimOut}
\MyIO


\begin{VerbatimOut}{z.out}


\section{Text}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{e.g.,}
\ix{e.g.}

``e.g.'' should always be followed by a comma.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{``et al.'' is an abbreviation}
\ix{et al.}

The phrase ``et al.''
is an abbreviation
and should always be followed by a period.
It should be in the normal font for your document---%
do not italicize or underline it.

Example:\\[6pt]
\indent\indent
\begin{tabular}{@{}ll@{}}
  input&   \verb+Thun et al.~used data from Santa Claus.+\\
  output&  Thun et al.~used data from Santa Claus.\\
  comment& my recommendation\\[6pt]
  input&   \verb+Thun et al. used data from Santa Claus.+\\
  output&  Thun et al. used data from Santa Claus.\\
  comment& too much space after period---\LaTeX\ thinks period is end of sentence\\[6pt]
  input&   \verb+Thun et al\@. used data from Santa Claus.+\\
  output&  Thun et al\@. used data from Santa Claus.\\
  comment& spacing is right but the ``et al.'' could occur at end of a line\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{i.e.,}
\ix{i.e.}

``i.e.'' should always be followed by a comma.
\end{VerbatimOut}

\MyIO


==> others/ap-computer-science.tex <==
\ProvidesFile{ap-computer-science.tex}[2021-08-23 computer science appendix]

\begin{VerbatimOut}{z.out}
\chapter{COMPUTER SCIENCE}
\ix{computer science//Computer Science appendix}

The cryptocode package \cite{mittelbach2020}
\ix{cryptocode//pseudocode//algorithm//protocol}
is used to typeset pseudocode,
algorithms,
and protocols.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Protocol examples}

\begin{protocol}[ht]
  \caption{This is the first protocol caption.}
  This is the first protocol.
\end{protocol}

\begin{protocol}[ht]
  \caption{This is the second protocol caption.}
  \pseudocodeblock
  {
    \textbf{Alice} \> \> \textbf{Bob}\\
    b \sample \bin \> \>\\
    \> \xrightarrow{\text{send over } b} \> \\
    \> \> \text{do something}
  }
\end{protocol}
\end{VerbatimOut}

\MyIO


==> others/ap-defining-commands.tex <==
\ProvidesFile{ap-defining-commands.tex}[2021-08-23 defining commands appendix]

\begin{VerbatimOut}{z.out}
\chapter{DEFINING COMMANDS}

The next paragraph demonstrates how to define and use a command.

\renewcommand{\t}[2]
{%
  Editors recommend that a #1 should never be
  followed by a #2 without some intervening text.
}

\t{chapter title}{section heading}
I suggest writing for readers.
Break the rules if necessary.

\end{VerbatimOut}

\MyIO


==> others/ap-electrical-engineering.tex <==
\ProvidesFile{ap-electrical-engineering.tex}[2021-08-23 electrical engineering appendix]

\begin{VerbatimOut}{z.out}
\chapter{ELECTRICAL ENGINEERING}
\ix{electrical engineering//Electrical Engineering appendix}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Amplifiers}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
This \qty{18}{\W} MOSFET amplifier
with npn transistor was done by Ram\'on Jaramillo
\cite{jaramillo}.
\ix{Jaramillo, Ram\'on}
This example make uses the \CircuiTikZLogo\index{\CircuiTikZLogo}
\cite{redaelli2021}
\ix{Redaelli, Massimo A.}%
and siunitx packages.

\begin{tikzpicture}[scale=2]
  \draw[color=black, thick]
    (0,0) to [short,o-] (6,0){} % Baseline for connection to ground
    % Input and ground
    (0,1) node[]{\large{\textbf{INPUT}}}
    % Connection of passive components
    (5,0) node[ground]{} node[circ](4.5,0){}
    (0,2) to [cC, l=$C_1$, o-] (0.5,2)
    to [R,l=$R_1$,](1.5,2)
    to node[short]{}(2.6,2)
    (1.5,2) to [C, l=$C_2$, *-] (1.5,3) -| (5,3)
    (2.2,2) to [R, l=$R_2$, *-*] (2.2,3)
    (2.2,3) to [cC, l=$C_3$, *-] (2.2,5) -| (3,5)
    % Transistor Bipolar Q1
    (3,0) to [R,l=$R_5$,-*] (3,1.5)
    to [Tnpn,n=npn1] (3,2.5)
    (npn1.E) node[right=3mm, above=5mm]{$Q_1$} % Labelling the NPN transistor
    (4,0) to [cC, l_=$C_4$, *-] (4, 1.5)--(3,1.5)
    (2.2,0) to [vR, l=$R_3$, *-*] (2.2,2)
    (3,2.5) to node[short]{}(3,3)
    (3,5) to [pR, n=pot1, l_=$R_4$, *-] (3,3)
    (3,5) to [R, l=$R_6$, *-] (5,5)
    to [short,*-o](5,5.5) node[right]{$V_S=40 V$}
    % Mosfet Transistors
    (5,3) to [Tnigfetd,n=mos1] (5,5)
    (mos1.B) node[anchor=west]{$Q_2$} % Labelling MOSFET Q2 Transistor
    (pot1.wiper) to [R, l=$R_7$] (4.5,4) -| (mos1.G)
    (5,1.5) to [Tpigfetd,n=mos2] (5,2.5)
    (5,0) to (mos2.S)
    (3,2.5) to [R, l=$R_8$, *-] (4.5,2.5)
    -| (mos2.G)
    (mos2.B) node[anchor=west]{$Q_3$} % Labelling MOSFET Q3 Transistor
    % Output
    (6,3) to [cC, l=$C_5$,-*](5,3)
    (6,3) to [short,-o] (6,2){}
    (mos1.S)--(mos2.D)
    (6,0) to [short,-o] (6,1){} node[above=7mm]{\large{\textbf{SPEAKER}}}
    ;
\end{tikzpicture}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Kalman Filter System Model}

This Kalman filter system model was done by Burkart Lingner
\cite{lingner2010}.
\ix{Lingner, Burkart}

% An example using TikZ/PGF 2.00
%
% Features: Decorations, Fit, Layers, Matrices, Styles
% Tags: Block diagrams, Diagrams
% Technical area: Electrical engineering

%%%% \documentclass[a4paper,10pt]{article}
%%%% 
%%%% \usepackage[english]{babel}
%%%% \usepackage[T1]{fontenc}
%%%% \usepackage[ansinew]{inputenc}
%%%% 
%%%% \usepackage{lmodern}	% font definition
%%%% \usepackage{amsmath}	% math fonts
%%%% \usepackage{amsthm}
%%%% \usepackage{amsfonts}
%%%% 
%%%% \usepackage{tikz}
%%%% 
%%%% %%%<
%%%% \usepackage{verbatim}
%%%% \usepackage[active,tightpage]{preview}
%%%% \PreviewEnvironment{tikzpicture}
%%%% \setlength\PreviewBorder{5pt}%
%%%% %%%>
%%%% 
%%%% \begin{comment}
%%%% :Title: Kalman Filter System Model
%%%% :Slug: kalman-filter
%%%% :Author: Burkart Lingner
%%%% 
%%%% This is the system model of the (linear) Kalman filter. 
%%%% 
%%%% \end{comment}
%%%% 
%%%% 

\begin{figure}[htbp]
\caption{Kalman filter system model}
\centering
% The state vector is represented by a blue circle.
% "minimum size" makes sure all circles have the same size
% independently of their contents.
\tikzstyle{state}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=blue!80,
                                    fill=blue!20]

% The measurement vector is represented by an orange circle.
\tikzstyle{measurement}=[circle,
                                                thick,
                                                minimum size=1.2cm,
                                                draw=orange!80,
                                                fill=orange!25]

% The control input vector is represented by a purple circle.
\tikzstyle{input}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=purple!80,
                                    fill=purple!20]

% The input, state transition, and measurement matrices
% are represented by gray squares.
% They have a smaller minimal size for aesthetic reasons.
\tikzstyle{matrx}=[rectangle,
                                    thick,
                                    minimum size=1cm,
                                    draw=gray!80,
                                    fill=gray!20]

% The system and measurement noise are represented by yellow
% circles with a "noisy" uneven circumference.
% This requires the TikZ library "decorations.pathmorphing".
\tikzstyle{noise}=[circle,
                                    thick,
                                    minimum size=1.2cm,
                                    draw=yellow!85!black,
                                    fill=yellow!40,
                                    decorate,
                                    decoration={random steps,
                                                            segment length=2pt,
                                                            amplitude=2pt}]

% Everything is drawn on underlying gray rectangles with
% rounded corners.
\tikzstyle{background}=[rectangle,
                                                fill=gray!10,
                                                inner sep=0.2cm,
                                                rounded corners=5mm]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]
    % "text height" and "text depth" are required to vertically
    % align the labels with and without indices.
  
  % The various elements are conveniently placed using a matrix:
  \matrix[row sep=0.5cm,column sep=0.5cm] {
    % First line: Control input
    &
        \node (u_k-1) [input]{$\mathbf{u}_{k-1}$}; &
        &
        \node (u_k)   [input]{$\mathbf{u}_k$};     &
        &
        \node (u_k+1) [input]{$\mathbf{u}_{k+1}$}; &
        \\
        % Second line: System noise & input matrix
        \node (w_k-1) [noise] {$\mathbf{w}_{k-1}$}; &
        \node (B_k-1) [matrx] {$\mathbf{B}$};       &
        \node (w_k)   [noise] {$\mathbf{w}_k$};     &
        \node (B_k)   [matrx] {$\mathbf{B}$};       &
        \node (w_k+1) [noise] {$\mathbf{w}_{k+1}$}; &
        \node (B_k+1) [matrx] {$\mathbf{B}$};       &
        \\
        % Third line: State & state transition matrix
        \node (A_k-2)         {$\cdots$};           &
        \node (x_k-1) [state] {$\mathbf{x}_{k-1}$}; &
        \node (A_k-1) [matrx] {$\mathbf{A}$};       &
        \node (x_k)   [state] {$\mathbf{x}_k$};     &
        \node (A_k)   [matrx] {$\mathbf{A}$};       &
        \node (x_k+1) [state] {$\mathbf{x}_{k+1}$}; &
        \node (A_k+1)         {$\cdots$};           \\
        % Fourth line: Measurement noise & measurement matrix
        \node (v_k-1) [noise] {$\mathbf{v}_{k-1}$}; &
        \node (H_k-1) [matrx] {$\mathbf{H}$};       &
        \node (v_k)   [noise] {$\mathbf{v}_k$};     &
        \node (H_k)   [matrx] {$\mathbf{H}$};       &
        \node (v_k+1) [noise] {$\mathbf{v}_{k+1}$}; &
        \node (H_k+1) [matrx] {$\mathbf{H}$};       &
        \\
        % Fifth line: Measurement
        &
        \node (z_k-1) [measurement] {$\mathbf{z}_{k-1}$}; &
        &
        \node (z_k)   [measurement] {$\mathbf{z}_k$};     &
        &
        \node (z_k+1) [measurement] {$\mathbf{z}_{k+1}$}; &
        \\
    };
    
    % The diagram elements are now connected through arrows:
    \path[->]
        (A_k-2) edge[thick] (x_k-1)	% The main path between the
        (x_k-1) edge[thick] (A_k-1)	% states via the state
        (A_k-1) edge[thick] (x_k)		% transition matrices is
        (x_k)   edge[thick] (A_k)		% accentuated.
        (A_k)   edge[thick] (x_k+1)	% x -> A -> x -> A -> ...
        (x_k+1) edge[thick] (A_k+1)
        
        (x_k-1) edge (H_k-1)				% Output path x -> H -> z
        (H_k-1) edge (z_k-1)
        (x_k)   edge (H_k)
        (H_k)   edge (z_k)
        (x_k+1) edge (H_k+1)
        (H_k+1) edge (z_k+1)
        
        (v_k-1) edge (z_k-1)				% Output noise v -> z
        (v_k)   edge (z_k)
        (v_k+1) edge (z_k+1)
        
        (w_k-1) edge (x_k-1)				% System noise w -> x
        (w_k)   edge (x_k)
        (w_k+1) edge (x_k+1)
        
        (u_k-1) edge (B_k-1)				% Input path u -> B -> x
        (B_k-1) edge (x_k-1)
        (u_k)   edge (B_k)
        (B_k)   edge (x_k)
        (u_k+1) edge (B_k+1)
        (B_k+1) edge (x_k+1)
        ;
    
    % Now that the diagram has been drawn, background rectangles
    % can be fitted to its elements. This requires the TikZ
    % libraries "fit" and "background".
    % Control input and measurement are labeled. These labels have
    % not been translated to English as "Measurement" instead of
    % "Messung" would not look good due to it being too long a word.
    \begin{pgfonlayer}{background}
        \node [background,
                    fit=(u_k-1) (u_k+1),
                    label=left:Entrance:] {};
        \node [background,
                    fit=(w_k-1) (v_k-1) (A_k+1)] {};
        \node [background,
                    fit=(z_k-1) (z_k+1),
                    label=left:Measure:] {};
    \end{pgfonlayer}
\end{tikzpicture}

\end{figure}
\end{VerbatimOut}

\MyIO


==> others/ap-figures.tex <==
\ProvidesFile{ap-figures.tex}[2021-08-23 figures appendix]

\begin{VerbatimOut}{z.out}
\chapter{FIGURES}

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The
\verb+h+
specifier used in all the examples below
tells \LaTeX\ to put the figure
``here''
instead of trying
to find a good spot
at the top or bottom of a page.
Specifiers can be combined,
for example,
``\verb+\begin{figure}[htbp!]+''.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The complete list of specifiers:
\vspace*{6pt}
\begin{center}
  \begin{tabular}{@{}ll@{}}
    \toprule
    \bf Specifier& \bf Description\\
    \midrule
    \noalign{\vspace*{2pt}}
    \tt b& bottom of page\\
    \tt h& here on page\\
    \tt p& on separate page of figures\\
    \tt t& top of page\\
    \tt !& try hard to put figure as early as possible\\
    \bottomrule
  \end{tabular}
\end{center}
\end{VerbatimOut}

\MyIO


% !!!! Label ``fi:not-centered'' is ``\ref{fi:not-centered}''.
% !!!! Label ``sf:four-parts-c'' is ``\ref{sf:four-parts-c}''.

\begin{VerbatimOut}{z.out}

% MyRepeat is defined in MyRepeat.sty.
\MyRepeat{This is the first paragraph.  }{5}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{figure}
  This is the figure.
  \caption{%
    Allocation to Common Edge for
    \(p(x_i) = 1-e^{-x_iz}\)% \frac{-x_i}z}\)%
  }
\end{figure}
\end{VerbatimOut}

\MyIO



\begin{VerbatimOut}{z.out}

\begin{figure}[ht]
  \includegraphics{gr-plot.pdf}
  \caption
  {%
    By default figures are not centered.
    This is a long caption to demonstrate that captions are single spaced.
    This is a long caption to demonstrate that captions are single spaced.%
  }
  \label{fi:not-centered}
\end{figure}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\MyRepeat{This is the second paragraph.  }{10}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{figure}[ht]
  \centering
  \includegraphics{gr-plot.pdf}
  \caption{Use {\tt \char'134centering\/} to center figures.}
  \label{fi:centered}
\end{figure}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\MyRepeat{This is the third paragraph.  }{15}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{figure}[ht]
  \centering
  \includegraphics{gr-plot.pdf}
  \caption{This is another figuure.}
  \label{fi:another}
\end{figure}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\MyRepeat{This is the fourth paragraph.  }{10}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
  
% See pages 4--5 of
%   http://mirrors.ibiblio.org/CTAN/macros/latex/contrib/caption/subcaption.pdf
% for how to use \subcaptionbox.
\begin{figure}[ht]
  % Center the entire figure (containing the two subfigures).
  \centering 
    % The \subcaptionbox for the first subfigure.
    \subcaptionbox
      % The first subcaption with a \label.
      % Use \ref{sf:two-parts-a} to print the subcaption number.
      {First subcaption.\label{sf:two-parts-a}}%
      % The first subfigure is this wide.
      [2in]%
      % This is the first subfigure.
      % You'll usually use an \includegraphics{filename}
      % inside the braces on the next line.
      {\bfseries First subfigure.}%
    % Put 0.5 inches of blank space between the subfigures.
    \hskip 0.5truein
    \subcaptionbox
      {Second subcaption.\label{sf:two-parts-b}}%
      [2in]%
      {\bfseries Second subfigure.}%
    % The caption for the entire figure (containing two subfigures).
    \caption{This figure has two parts.}
    % The label for the entire figure.
    \label{fi:two-parts}
\end{figure}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\MyRepeat{This is the fifth paragraph.  }{10}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
  
\newpage

\begin{figure}[ht]
  \centering
    \subcaptionbox
      {First subcaption.\label{sf:four-parts-a}}
      [2in]%
      {\bfseries First subfigure.}%
    \hskip 0.5truein
    \subcaptionbox
      {Second subcaption.\label{sf:four-parts-b}}
      [2in]%
      {\bfseries Second subfigure.}%
    \vspace*{\baselineskip}
    \subcaptionbox
      {Third subcaption.\label{sf:four-parts-c}}
      [2in]%
      {\bfseries Third subfigure.}%
    \hskip 0.5truein
    \subcaptionbox
      {Fourth subcaption.\label{sf:four-parts-d}}
      [2in]%
      {\bfseries Fourth subfigure.}%
  \caption{This figure has four parts.}
  \label{fi:four-parts}
\end{figure}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\MyRepeat{This is the sixth paragraph.  }{10}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\newpage

\begin{figure}[ht]
  \centering 
    % Use a 5" font.
    {\fontsize{5in}{5in}\selectfont\(\hspace*{-0.07em}\sqrt 2\)}
    \caption{%
      A big ``\(\sqrt 2\)''.
      \LaTeX\ can make output big enough for T-shirts or posters.
      Square roots are printed with space before them,
      I put some negative horizontal space before this one to center it.%
    }
\end{figure}
\end{VerbatimOut}

\MyIO


\begin{figure}
  This is the figure.
  \caption{%
    Allocation to Common Edge for
    \(p(x_i) = 1-e^{-x_iz}\)% \frac{-x_i}z}\)%
  }
\end{figure}

\begin{VerbatimOut}{z.out}

\newpage

The remainder of this file tests having lots of figures.
There are 20 figures in this test.

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-01.pdf}
  \caption{Test figure 1 of 20.}
  \label{fi:1of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-02.pdf}
  \caption{Test figure 2 of 20.}
  \label{fi:2of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-03.pdf}
  \caption{Test figure 3 of 20.}
  \label{fi:3of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-04.pdf}
  \caption{Test figure 4 of 20.}
  \label{fi:4of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-05.pdf}
  \caption{Test figure 5 of 20.}
  \label{fi:5of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-06.pdf}
  \caption{Test figure 6 of 20.}
  \label{fi:6of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-07.pdf}
  \caption{Test figure 7 of 20.}
  \label{fi:7of20centered7}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-08.pdf}
  \caption{Test figure 8 of 20.}
  \label{fi:8of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-09.pdf}
  \caption{Test figure 9 of 20.}
  \label{fi:9of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-10.pdf}
  \caption{Test figure 10 of 20.}
  \label{fi:10of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-11.pdf}
  \caption{Test figure 11 of 20.}
  \label{fi:11of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-12.pdf}
  \caption{Test figure 12 of 20.}
  \label{fi:12of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-13.pdf}
  \caption{Test figure 13 of 20.}
  \label{fi:13of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-14.pdf}
  \caption{Test figure 14 of 20.}
  \label{fi:14of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-15.pdf}
  \caption{Test figure 15 of 20.}
  \label{fi:15of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-16.pdf}
  \caption{Test figure 16 of 20.}
  \label{fi:16of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-17.pdf}
  \caption{Test figure 17 of 20.}
  \label{fi:17of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-18.pdf}
  \caption{Test figure 18 of 20.}
  \label{fi:18of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-19.pdf}
  \caption{Test figure 19 of 20.}
  \label{fi:19of20}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{gr-tally-20.pdf}
  \caption{Test figure 20 of 20.}
  \label{fi:20of20}
\end{figure}
\end{VerbatimOut}

\MyIO


==> others/ap-frequently-asked-questions.tex <==
\ProvidesFile{ap-frequently-asked-quetions.tex}[2021-08-23 Frequently Asked Questions appendix]

\begin{VerbatimOut}{z.out}
\chapter{FREQUENTLY ASKED QUESTIONS}
\ix{frequently asked questions//Frequently Asked Questions appendix}

{\bfseries PART OF THESIS WITH PROBLEM}

{
  \def\part#1%
  {
    \vspace*{\baselineskip}
    {\bfseries #1}
  }

  \def\qa#1#2%
  {
    \vspace*{\baselineskip}
    {\small\bfseries Q}: #1\endgraf
    \vspace*{0.5\baselineskip}
    {\small\bfseries A}: #2\endgraf
  }


  \part{Entire Thesis}

  \qa
  {What \LaTeX\ comand should I use to compile my thesis?}
  {%
    The \LuaLaTeXLogo%
    \ix{LuaLaTeX//lualatex}%
    \index{\LuaLaTeXLogo}
    program in the \TeXLiveLogo%
    \index{\TeXLiveLogo}%
    \ix{TeX Live}
    software distribution.
    Overleaf \cite{overleaf}
    (run \LaTeX%
    \index{\LaTeX}
    over the web)
    uses \TeXLiveLogo---%
    in Overleaf click {\tt Menu\/} key in upper left corner of window
    and set {\tt Compiler\/} to {\tt LuaLaTeX} to run \LuaLaTeXLogo.)
    \TeXLiveLogo\ runs on Linux\ix{Linux},
    MacOS\ix{MacOS},
    Unix\ix{Unix},
    and Windows\ix{Windows}.%
  }


  \part{References}

  \qa
  {URLs are not getting printed.  What should I do?}%
  {Make sure you are processing your docuent with \LuaLaTeXLogo.}
}
\end{VerbatimOut}

\MyIO


==> others/ap-graphics.tex <==
\ProvidesFile{ap-graphics.tex}[2021-08-23 graphics appendix]

\begin{VerbatimOut}{z.out}
\chapter{GRAPHICS}

There are many ways to make graphics for \LaTeX.
I like to use a system that uses \LaTeX\ fonts
so the appearance of the output is more professional.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{\LaTeX\ \TikZLogo\ package}
\index{TikZ@\TikZLogo}  
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\subsection{Yin and yang}

This Yin and yang example was done by Thomas G. Kristensen \cite{kristensen}.
This is the ``traditional Taijitu symbol from Chinese philosophy''.\\
\ix{Kristensen, Thomas G.//Taijitu symbol//Yin and yang symbol}

\index{TikZ@\TikZLogo}  
\begin{tikzpicture}
  % Yin and yang
  % Author: Thomas G. Kristensen
  
  % color one half of a unit circle                                              
  \begin{scope}
    \clip (0,0) circle (1cm);
    \fill[black] (0cm,1cm) rectangle (-1cm, -1cm);
  \end{scope}

  % fill heads                                                                   
  \fill[black] (0,0.5) circle (0.5cm);
  \fill[white] (0,-0.5) circle (0.5cm);

  % fill eyes                                                                    
  \fill[white] (0,0.5) circle (0.1cm);
  \fill[black] (0,-0.5) circle (0.1cm);

  % outer line                                                                   
  \draw (0,0) circle (1cm);

\end{tikzpicture}
\end{VerbatimOut}

\MyIO



\begin{VerbatimOut}{z.out}

\section{Mathematica (which uses Wolfram Language)}
\ix{Mathematica}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{MATLAB}
\ix{MATLAB}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{\protect\METAPOSTLogo\ (uses \LaTeX\ fonts)}
\index{METAPOST@\METAPOSTLogo}  

I did these \METAPOSTLogo\ \cite{metapost} examples
for Yanghyun Kim \cite{kim2009}.
\ix{Kim, Yanghyun}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\includegraphics{gr-kim1.pdf}
\todoerror{need source code}  

\vspace{0.1truein}

\includegraphics{gr-kim2.pdf}
\todoerror{need source code}  
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{\METAPOSTLogo\ Tally Example}
\label{ss:tally-example}

Whenever I use files with numbers in them I like to put leading zeros
in the names so they will be listed in order in the directory.

These 20 graphics (gr-tally-01.pdf through gr-tally-20.pdf)

\vspace*{6pt}

{%
  % Let * represent zero or more spaces!
  % Method 1: \def\g#1{ requires using \g*{10} for 10.
  %           Two shifted characters, { and } are needed.
  % Method 2: \def\g#1/{ requires using \g*10/ for 10.
  %           One unshifted character, / is needed.
  \def\g#1/{\includegraphics[scale=0.5]{gr-tally-#1.pdf}}%

  % Note that tabular* instead of tabular is used below.
  %   The {\textwidth} makes the total width of the table the width
  % of the printed area of the page.
  %   The @{\kern2\parindent} puts blank space the width of two
  % paragraph indents before the first column.
  %   The @{extracolsep{\fill}} adds \fill space between all subsequent
  % columns.
  %   The lll left justifies the next three columns.
  % after the column.
  %   The @{\kern2\parindent} puts blank space the width of two
  % paragraph indents before the first column.
  \begin{tabular*}{\textwidth}{@{\kern2\parindent}@{\extracolsep{\fill}}lll@{\kern2\parindent}}%
    \g 01/& \g 02/& \g 03/\\
    \g 04/& \g 05/& \g 06/\\
    \g 07/& \g 08/& \g 09/\\
    \g 10/& \g 11/& \g 12/\\
    \g 13/& \g 14/& \g 15/\\
    \g 16/& \g 17/& \g 18/\\
    \g 19/& \g 20/\\
  \end{tabular*}%
}
\noindent were produced by

\MyI{misc/tally.mp}

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{R}
\ix{R}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{\TikZLogo\ and PGF (uses \LaTeX\ fonts)}
\index{TikZ@\TikZLogo}
\ix{PGF}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Clock}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The idea for this clock was originally
from a Google+ posting by
Afamefuna ``Ferdy'' Ibeabuchia.  \ix{Ibeabuchia, Afamefuna ``Ferdy''//PGF}
\index{TikZ@\TikZLogo}

\hbox to\textwidth{%
  \hfil
  \begin{tikzpicture}
    \def\CenterRadius{0.04cm}
    \def\InnerTickRadius{3.6cm}
    \def\OuterTickRadius{3.8cm}
    % Make \LR be an abbreviation for \LabelRadius so the
    % lines below will fit within the width of the page.
    \def\LabelRadius{4.5cm}      \let\LR=\LabelRadius
    \def\HourHandRadius{2.5cm}   \def\HourHandBase{0.3cm}
    \def\MinuteHandRadius{3cm}   \def\MinuteHandBase{0.4cm}
    \def\SecondHandRadius{3.5cm} \def\SecondHandBase{0.5cm}
    \def\DS{\displaystyle}
    \fill (0,0) circle (\CenterRadius);
    \foreach \i in {0,30,...,330}
    \draw (\i:\InnerTickRadius)--(\i:\OuterTickRadius);
    \node at (  0:\LR) {$\DS \qquad \sqrt9 + 9 - 9$};        %  3
    \node at ( 30:\LR) {$\DS \frac{9+9}9$};                  %  2
    \node at ( 60:\LR) {$\DS \frac{\sqrt9\sqrt9}9$};         %  1
    \node at ( 90:\LR) {$\DS 9 + \frac9{\sqrt9}$};           % 12
    \node at (120:\LR) {$\DS \frac{99}9$};                   % 11
    \node at (150:\LR) {$\DS 9 + \frac99$};                  % 10
    \node at (180:\LR) {$\DS \sqrt[\scriptstyle 9]{9^9}$};   %  9
    \node at (210:\LR) {$\DS 9 - \frac99$};                  %  8
    \node at (240:\LR) {$\DS 9 - \sqrt9 + \lceil.9\rceil$};  %  7
    \node at (270:\LR) {$\DS 9 - \frac9{\sqrt9}$};           %  6
    \node at (300:\LR) {$\DS \sqrt9\,! - \frac99$};          %  5
    \node at (330:\LR) {$\DS \sqrt9 + \frac99$};             %  4
    % In the following
    %   ABBREVIATION    DESCRIPTION
    %   deg             degrees
    %   min             minutes
    %   sec             seconds
    % for second hand:
    %   (9 sec/60 sec) * 360 deg = 54 deg;
    %   90 deg - 54 deg = 36 deg
    \draw[rotate around={36:(0,0)}]
      (-\SecondHandBase,\SecondHandBase) -- (\SecondHandRadius,0)
        -- (-\SecondHandBase,-\SecondHandBase) -- cycle;
    % for minute hand:
    %   (9 min/60 min) * 360 deg = 54 deg;
    %   90 deg - 54 deg = 36 deg
   \draw[rotate around={36:(0,0)}]
     (-\MinuteHandBase,\MinuteHandBase) -- (\MinuteHandRadius,0)
       -- (-\MinuteHandBase,-\MinuteHandBase) -- cycle;
    % for hour hand:
    %   (9 min * (60 sec/1 min)) + 9 sec) / 3600 sec
    %     = 549 sec / 3600 sec = 0.1525
    %   The hour hand is 0.1525 of the way from 9:00 to 10:00.
    %   Each hour is 30 degrees on the clock, so the hour hand
    %   position is
    %     30 deg * 0.1525 = 4.575 deg past 9:00
    %   180 deg - 4.575 deg = 175.425 deg
    \draw[rotate around={175.425:(0,0)}]
      (-\HourHandBase,\HourHandBase) -- (\HourHandRadius,0)
      -- (-\HourHandBase,-\HourHandBase) -- cycle;
  \end{tikzpicture}
  \hfil
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Glider}
\ix{Hirzel, Alex//Glider emblem representing the hacker community}

The glider
is a pattern from the Game of Life,
and it's used as an emblem representing the hacker community.

\begin{tikzpicture}[thick]
  \draw (0,0) grid (3,3);
  \foreach \c in {(0,0), (1,0), (2,0), (2,1), (1,2)}
    \fill \c + (0.5,0.5) circle (0.42);
\end{tikzpicture}
\end{VerbatimOut}

\MyIO


==> others/ap-linguistics.tex <==
\ProvidesFile{ap-linguistics.tex}[2021-08-23 linguistics appendix]

\begin{VerbatimOut}{z.out}
\chapter{LINGUISTICS}
\ix{linguistics//Linguistics appendix}

See WIKIBOOKS \LaTeX/Linguistics \cite{wikibooks-latex-linguistics}
or google for the information you need.

The doulossil font \cite{tambe2020}
is a TrueType font.
Version 0.1 on September 21, 2020 claimed
``it has characters that are not in other TeX IPA fonts''.
\end{VerbatimOut}

\MyIO


==> others/ap-mathematics.tex <==
\ProvidesFile{ap-mathematics.tex}[2021-08-23 mathematics appendix]

\begin{VerbatimOut}{z.out}
\chapter{MATHEMATICS}
\ix{mathematics//Mathematics appendix}

\PurdueThesisLogo\ loads the \AMSmathLogo\ package \cite{amslatex3project2019}
to do mathematics.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
There are two types of mathematics in \LaTeX.
Text math is math that that is interspersed with text.
For example, this is text math: \(a = b + c\).
This is display math:
\begin{equation}
  a = b + c
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\newpage

\section{Standard Functions}

Standard functions should be in a roman font.
Like this: \(\cos\theta\).
Here is a list of standard function commands:\\

% The "@{\hspace*{\parindent}}" indents the table
% the same amount as a paragraph.
\begin{tabular}{@{\hspace*{\parindent}}llll@{}}
  \verb+\arccos+& \verb+\csc+& \verb+\ker+&    \verb+\min+\\
  \verb+\arcsin+& \verb+\deg+& \verb+\lg+&     \verb+\Pr+\\
  \verb+\arctan+& \verb+\det+& \verb+\lim+&    \verb+\sec+\\
  \verb+\arg+&    \verb+\dim+& \verb+\liminf+& \verb+\sin+\\
  \verb+\cos+&    \verb+\exp+& \verb+\limsup+& \verb+\sinh+\\
  \verb+\cosh+&   \verb+\gcd+& \verb+\ln+&     \verb+\sup+\\
  \verb+\cot+&    \verb+\hom+& \verb+\log+&    \verb+\tan+\\
  \verb+\coth+&   \verb+\inf+& \verb+\max+&    \verb+\tanh+\\
\end{tabular}
\ix
{%
  arccos//arcsin//arctan//arg//cos//cosh//cot//coth%
  //csc//deg//det//dim//exp//gcd//hom//inf%
  //ker//lg//lim//liminf//limsup//ln//log//max%
  //min//Pr//sec//sin//sinh//sup//tan//tanh%
}
\index{\verb+\arccos+} \index{\verb+\arcsin+} \index{\verb+\arctan+} \index{\verb+\arg+}
\index{\verb+\cos+} \index{\verb+\cosh+} \index{\verb+\cot+} \index{\verb+\coth+}
\index{\verb+\csc+} \index{\verb+\deg+} \index{\verb+\det+} \index{\verb+\dim+}
\index{\verb+\exp+} \index{\verb+\gcd+} \index{\verb+\hom+} \index{\verb+\inf+}
\index{\verb+\ker+} \index{\verb+\lg+} \index{\verb+\lim+} \index{\verb+\liminf+}
\index{\verb+\limsup+} \index{\verb+\ln+} \index{\verb+\log+} \index{\verb+\max+}
\index{\verb+\min+} \index{\verb+\Pr+} \index{\verb+\sec+} \index{\verb+\sin+}
\index{\verb+\sinh+} \index{\verb+\sup+} \index{\verb+\tan+} \index{\verb+\tanh+}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\newpage

\section{English Words in Math}

English words in math should be in a roman font like this:\\
Let the maximum value of \(a\) be \(a_\text{max}\).\\
\(a_\text{max} \ge a_\text{min}\) should always be true.\\
The temperature in the attic is \(t_\text{attic}\).
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\section{Text Math}

Use \verb+\(+ to start text math and \verb+\)+ to end text math.
Some people use \verb+$+ to start and end text math---I don't
recommend that because \LaTeX\ can give better error messages
if you use \verb+\(+ and \verb+\)+.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\section{Displayed Equations}

Do not use \verb+$$+ to start or end displayed math like \TeX\ uses
\cite{gratzer2016}.

The \AMSmathLogo\ package provides a number
of additional displayed equation structures
beyond the ones provided in basic \LaTeX.
The augmented set includes \cite{amslatex3project2019b}:

\hbox to\hsize{%
  \hss
  \begin{tabular}{@{}ll@{}}
    \toprule
    \bfseries Environment& \bfseries Used for\\
    \midrule
    \tt equation& used for single equations\\
    \tt multline& split single equations over multiple lines\\
    \tt gather& collect but do not align multiple equations\\
    \tt align& align multiple equations\\
    \tt alignat& aligns multiple equations at multiple places\\
    \tt flalign& aligns multiple equations at multiple places on full length lines\\
    \tt split& split a single equation over multiple lines\\
    \bottomrule
  \end{tabular}%
  \hss
}

All but \verb+split+ can be followed by \verb+*+ to not number equations.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{\texttt{equation} environment}

The \verb+equation+ environment is used for single equations.

\begin{equation}
  E = mc^2
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The \verb+equation*+ environment does single, unnumbered equations.

\begin{equation*}
  a = b_0c + \frac12 de^2 + {\textstyle \frac12} fg^2
    + h_1 + h_2 + \cdots + h_n
    \qquad \text{for \(c \ne d\) and \(g < \infty\)}
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\textcite{greene-2021-03-14} wrote
% \begin{quotation}  
  For
  \href{https://twitter.com/hashtag/PiDay?src=hashtag\_click\#PiDay}{\#PiDay},
  one of the coolest formulae for today's honoree:
  \[
    \frac 1\pi
    =
    \frac {\sqrt8} {9801}
    \sum_{n=0}^\infty
    \frac  {(4n!) (1103+26390n)}  {(n!)^4 396^{4n}}
  \]
% \end{quotation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

International standard ISO 80000-2:2019 \cite{iso8000022019}
states that $\mit e$,~$\mit i$,~$\mit j$,
and $\itpi$ should appear as
$e$,~$i$,~$j$
and~$\pi$ because they are constants.
This is done automatically by the pa-mismath package
that is loaded by thesis.tex.
See thesis.tex for more information,
including what to do if you're not using those as constants.

Euler's identity is
\begin{equation*}
  e^{i\pi} + 1 = 0.
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Here's a simple formula relating $e$,~$i$,~$\pi$, and~$\phi$,
the golden ratio
\begin{equation}
  e^{i\pi} + 2\phi = \sqrt 5.
\end{equation}
I didn't notice anything on the web about putting the symbol for
the golden ratio in a special font even though it is a constant.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

International standard ISO 80000-2:2019 \cite{iso8000022019}
states that the ``$d\/$'' in math differentials
should be typeset as ``$\di$''.
So,
\begin{equation*}
  \text{use } \int x\di x\qquad\qquad \text{instead of } \int x\,dx
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The formula for Bekenstein-Hawking entropy:

\begin{equation*}
  S_\text{BH}
  =
  \frac A {4L_P^2}
  = \frac {c^3A} {4G\hbar}
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Type in the math and let \LaTeX\ worry about the spacing.
You only need to do fine tuning by hand if it looks bad.

Another \verb+equation*+ environment,
note the spacing before the large close parenthesis:

\begin{equation*}
  \frac ab
    = ab^{-1}
    % Parens are the wrong size.
    = (\sqrt{\frac ab})^2
    % Parens are the right size but closing paren is too close to radical.
    = \left( \sqrt\frac ab \right)^2
    % Parens are right size but a negative thin space puts closing paren on top of radical.
    = \left( \sqrt\frac ab \!\right)^2
    % Parens are right size but a thin space puts closing paren too close to radical.
    = \left( \sqrt\frac ab \,\right)^2
    % Parens are right size but a medium space puts closing paren too close to radical.
    = \left( \sqrt\frac ab \:\right)^2
    % Parens are right size and I think a thick space looks the best.
    = \left( \sqrt\frac ab \;\right)^2
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{equation*}
  (\cos x)^2 + (\sin x)^2 = \cos^2 x + \sin^2 x = 1
\end{equation*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{equation}
  x \mod 2 =
  \begin{cases}
    0& \text{if $x$ is even}\\
    1& \text{if $x$ is odd}\\
  \end{cases}
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The first six derivatives of distance are velocity, acceleration, jerk, snap, crackle,
and pop \cite{reid2013}.

\begin{equation}
  % Every array element should be in \displaystyle (a big font).
  \AtBeginEnvironment{array}{\everymath{\displaystyle}}
  % Set space between columns to zero, use {} = ... to add a little space before the = "by hand".
  \arraycolsep = 0pt
  \text{distance derivitives} = \left\{\ %
    \begin{array}{llllllll}
      % I'm formatting the first 4 lines different from the last 3 so this will fit on one page.
      x&      {}=\text{distance}&     {}=vt\\[2pt]
      v&      {}=\text{velocity}&     {}=\frac{\di x}{\di t}\\[9pt]
      a&      {}=\text{acceleration}& {}=\frac{\di v}{\di t}& {}=\frac{\di^2x}{\di t^2}\\[9pt]
      \mit j& {}=\text{jerk}&         {}=\frac{\di a}{\di t}& {}=\frac{\di^2v}{\di t^2}&
        {}=\frac{\di^3x}{\di t^3}\\[9pt]
      s
        & {}=\text{snap}
        & {}=\frac{\di \mit j}{\di t}
        & {}=\frac{\di^2a}{\di t^2}
        & {}=\frac{\di^3v}{\di t^3}
        & {}=\frac{\di^4x}{\di t^4}\\[9pt]
      c
        & {}=\text{crackle}
        & {}=\frac{\di s}{\di t}
        & {}=\frac{\di^2\mit j}{\di t^2}
        & {}=\frac{\di^3a}{\di t^3}
        & {}=\frac{\di^4v}{\di t^4}
        & {}=\frac{\di^5x}{\di t^5}\\[9pt]
      p
        & {}=\text{pop}
        & {}=\frac{\di c}{\di t}
        & {}=\frac{\di^2s}{\di t^2}
        & {}=\frac{\di^3\mit j}{\di t^3}
        & {}=\frac{\di^4a}{\di t^4}
        & {}=\frac{\di^5v}{\di t^5}
        & {}=\frac{\di^6x}{\di t^6}
    \end{array}
  \right.
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{\texttt{multline} environment}

The \verb+multline+ environment is used
to split single equations over multiple lines.

\begin{multline}
  S = a + b + c + d + e + f + g + h + i + j\\
  + k + l + m + n + o + p\\
  + q + r + s + t + u + v + w + x + y + z
\end{multline}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{multline}
  S = a + b + c + d + e\\
  + f + g + h + i + j\\
  + k + l + m + n + o\\
  + p + q + r + s + t\\
  + u + v + w + x + y\\
  + z
\end{multline}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% Calculate width of space before equation plus equation number.
% (All digits are the same width.)
\newdimen{\tdimen}
\settowidth{\tdimen}{\kern\multlinetaggap (L.5)}
\begin{multline}
  S = a + b + c + d + e\\
  \makebox[\textwidth]{\hfill $+ f + g + h + i + j$\hfill\hfill\hfill\hfill\kern\tdimen}\\
  \makebox[\textwidth]{\hfill\hfill${} + k + l + m + n + o$\hfill\hfill\hfill\kern\tdimen}\\
  \makebox[\textwidth]{\hfill\hfill\hfill${} + p + q + r + s + t$\hfill\hfill\kern\tdimen}\\
  \makebox[\textwidth]{\hfill\hfill\hfill\hfill${} + u + v + w + x + y$\hfill\kern\tdimen}\\
  + z
\end{multline}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{\texttt{gather} environment}

The \verb+gather+ environment collects but does not align multiple equations.

\begin{gather}
  a = b + c + d + e + f + g + h + i + j + k + l\\
  m = n + o + p + q + r + s + t + u + v + w + x + y + z
\end{gather}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{gather}
  a = b + c + d + e + f + g + h + i + j + k + l\notag\\
  m = n + o + p + q + r + s + t + u + v + w + x + y + z
\end{gather}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{gather*}
  \alpha = \beta + \gamma + \delta + \eta\\
  \theta = \iota + \kappa + \lambda + \mu + \nu + \rho + \tau
\end{gather*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{gather}
  x_\text{min} + x_\text{max} \le \sum_{i=1}^n x_i\\
  x_\text{min} + x_\text{max}
    = \sum_{i=1}^n x_i - \sum_{i=2}^{n-1} x_i\quad\text{if $x$ is sorted}\\
  x_\text{min} \le \left(\sum_{i=1}^n x_i\right) / n
\end{gather}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{\texttt{align} environment}

The \verb+align+ environment aligns multiple equations.

\begin{align}
  a &= b + c + d\\
  e &= f + g + h + i + j
\end{align}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\begin{align}
  x = \frac{-b \pm \sqrt{b^2-4ac}}{2a}\notag\\
  % Put a thin space before the b^2 to improve the appearance.
  x = \frac{-b \pm \sqrt{\,b^2-4ac}}{2a}
\end{align}
\end{VerbatimOut}
\ix{align environment}
\index{\verb+\begin{align}+}
\ix{thin space}
\index{\verb+\,+}

\MyIO


\begin{VerbatimOut}{z.out}

Quadratic formula proof \cite{khan}:
\ix{quadratic formula}

% The align environment requires the amsmath package.
% Use \addtolength{\jot}{6pt} to increase the space between rows in an amsmath multi-line math formula.
% That's not done here so everything will fit on one page.
\begin{align}
  ax^2 + bx + c &= 0\\
  ax^2 + bx &= -c\notag\\
  % The "\," adds a thinspace of horizontal space.
  x^2 + \frac ba\,x &= -\frac ca\notag\\
  x^2 + \frac ba\,x + \frac{b^2}{4a^2} &= \frac{b^2}{4a^2} - \frac ca\notag\\
  \left(x + \frac b{2a}\right)^2 &= \frac{b^2}{4a^2} - \frac ca\notag\\
  \left(x + \frac b{2a}\right)^2 &= \frac{b^2}{4a^2} - \frac{4ac}{4a^2}\notag\\
  \left(x + \frac b{2a}\right)^2 &= \frac{b^2-4ac}{4a^2}\notag\\
  \sqrt{\left(x + \frac b{2a}\right)^2}
    &= \sqrt{\left(\frac{b^2-4ac}{4a^2}\right)}\notag\\
  x + \frac b{2a} &= \pm \frac{\sqrt{\,b^2-4ac}}{\sqrt{4a^2}}\notag\\
  x + \frac b{2a} &= \pm \frac{\sqrt{\,b^2-4ac}}{2a}\notag\\
  x &= - \frac b{2a} \pm \frac{\sqrt{\,b^2-4ac}}{2a}\notag\\
  x &= \frac{-b \pm \sqrt{\,b^2-4ac}}{2a}
\end{align}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{\texttt{alignat} environment}
\index{\verb+\begin{aligo}+@\verb+\begin{alignat}+}
\ix{alignat environment}

The \verb+alignat+ environment aligns multiple equations at multiple places.
\begin{alignat}{2}
  a &= b& \qquad\qquad& \text{set $a$}\\
  c &= d& &             \text{you guessed it, set $c$}\notag\\
  g &= h& &             \text{and finally, set $g$}
\end{alignat}
\index{\verb+\begin{aligo}+@\verb+\begin{alignat}+}
\ix{alignat environment}
  
I like to align input columns on the input if possible
and will sometimes use windows over~250 characters wide to do so.
If that won't work I sometimes do,
for example,
\begin{alignat}{2}
  a
    &= b
    & \qquad\qquad
    & \text{set $a$}\\
  c
    &= d
    &
    &\text{you guessed it, set $c$}\notag\\
  g
    &= h
    &
    &\text{and finally, set $g$}
\end{alignat}
\index{\verb+\begin{aligo}+@\verb+\begin{alignat}+}
\ix{alignat environment}

Do whatever works best for you.

\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Quadratic formula proof \cite{khan}:

% Make changes to \jot be local to the group that starts on the next line.
{
  % Increase distance between lines by 6pt.
  \addtolength{\jot}{6pt}
  \begin{alignat}{2}
    ax^2 + bx + c
      &= 0
      &
      &\text{subtract $c$}\\
    ax^2 + bx
      &= -c
      &
      &\text{divide by $a$}\notag\\
    % The "\," adds a thinspace of horizontal space.
    x^2 + \frac ba\,x
      &= -\frac ca
      &
      &\text{add $\displaystyle\frac{b^2}{4a^2}$}\notag\\
    x^2+\frac ba\,x+\frac{b^2}{4a^2}
      &= \frac{b^2}{4a^2}-\frac ca
      &
      &\text{factor left hand side}\notag\\
    \left(x+\frac b{2a}\right)^2
      &= \frac{b^2}{4a^2}-\frac ca
      &
      &\text{multiply right-most term by $\displaystyle\frac{4a}{4a}$}\notag\\
    \left(x + \frac b{2a}\right)^2
      &= \frac{b^2}{4a^2}-\frac{4ac}{4a^2}
      &
      &\text{use common denominator}\notag\\
    \left(x + \frac b{2a}\right)^2
      &= \frac{b^2-4ac}{4a^2}
      &
      &\text{take square root of each side}\notag\\
    \sqrt{\left(x + \frac b{2a}\right)^2}
      &= \sqrt{\left(\frac{b^2-4ac}{4a^2}\right)}
      &
      &\text{compute square root of each side}\notag\\
    x + \frac b{2a}
      &= \pm \frac{\sqrt{\,b^2-4ac}}{\sqrt{4a^2}}
      &
      &\text{simplify right hand denominator}\notag\\
    x + \frac b{2a}
      &= \pm \frac{\sqrt{\,b^2-4ac}}{2a}
      &
      &\text{subtract $\displaystyle\frac b{2a}$ from each side}\notag\\
    x
      &= -\frac b{2a} \pm \frac{\sqrt{\,b^2-4ac}}{2a}
      &\qquad
      &\text{use common denominator}\notag\\
    x
      &= \frac{-b \pm \sqrt{\,b^2-4ac}}{2a}
  \end{alignat}
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\index{\verb+\begin{flalign}+}
\todoindex{Verb+Begin-Ocurly-flalign-Ccurly+}
\ix{falign environment}
\subsection{\texttt{flalign} environment}

The \verb+flalign+ environment aligns multiple equations at multiple places
on full length lines.

\begin{flalign}
  a &= b&   &   & u &= v\\
  c &= d& m &= n& w &= x\notag\\
  g &= h&   &   & y &= z
\end{flalign}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\index{\verb+\begin{split}+}
\todoindex{Verb+Begin-Ocurly-split-Ccurly+}
\ix{split environment}
\subsection{\texttt{split} environment}

The \verb+split+ environment ???.
\end{VerbatimOut}

\MyIO
\index{\verb+\begin{split}+}
\todoindex{Verb+Begin-Ocurly-split-Ccurly+}
\ix{split environment}


\begin{VerbatimOut}{z.out}
\section{Theorem-like environments}

These theorem-like environments are defined
in the amsthm package or in\\  % break line here so we don't go past right margin
\verb+PurdueThesis.cls+.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\index{\verb+\begin{definition}+}
\todoindex{Verb+Begin-Ocurly-definition-Ccurly+}
\ix{definition environment}
\begin{definition}
  This is an example definition.
\end{definition}

\index{\verb+\begin{observation}+}
\todoindex{Verb+Begin-Ocurly-observation-Ccurly+}
\ix{observation environment}
\begin{observation}
  This is an example observation.
\end{observation}

\index{\verb+\begin{proof}+}
\todoindex{Verb+Begin-Ocurly-proof-Ccurly+}
\ix{proof environment}
\begin{proof}
  This is an example proof.
  If \(a = b\) and \(b = c\) then \(a = c\).
\end{proof}

\index{\verb+\begin{proposition}+}
\todoindex{Verb+Begin-Ocurly-proposition-Ccurly+}
\ix{proposition environment}
\begin{proposition}
  This is an example proposition.
\end{proposition}

\index{\verb+\begin{theorem}+}
\todoindex{Verb+Begin-Ocurly-theorem-Ccurly+}
\ix{theorem environment}
\begin{theorem}
  This is an example theorem.
\end{theorem}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Examples}

\subsection{Bayes' Theorem}
\ix{Bayes' Theorem}

Bayes' Theorem \cite{bayes}:
{
  \UndefineShortVerb{\|}
\[
  \text{P}(\text A|\text B)
    % The "\," puts a thin horizontal space there, 1/6 of an "em".
    % An "em" is roughly the width of a lowercase "m".
    = \frac{\text P(\text B|\text A)\,\text P(\text A)}{\text P(\text B)}
\]
}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Nicomachus's theorem}
\ix{Nicomachus's theorem}

Nicomachus's theorem \cite{wikipedia-nicomachus} states that
the sum of the first~$n$ cubes is the square of the~$n$th triangular number.
That is,
\[
  1^3 + 2^3 + 3^3 + \cdots + n^3 = (1 + 2 + 3 + \cdots + n)^2.
\]
The same equation may be written more compactly using the mathematical notation for summation:
\[
  \sum_{k=1}^n k^3 = \left(\sum_{k=1}^n k\right)^2.
\]
Also see the diagram on that web page.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Prime Number Theorem}
\ix{Prime Number Theorem}

\textcite{li2013} suggested using a functional equation
from the Prime Number Theorem proof
as an example:
\begin{equation}
  \int_1^x
    \sum_{p\le u}
    \left\lfloor\frac{\log u}{\log p}\right\rfloor
    \log p
    \,\text{d}u
    =
    \frac1{2\pi i}
    \int_{c-i\infty}^{c+i\infty}
    \frac{x^{s+1}}{s(s+1)}
    \left(-\frac{\zeta'(s)}{\zeta(s)}\right)
    \text{d}s
\end{equation}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\subsection{Quantum Mechanics}
\ix{Quantum Mechanics}

\textcite{greene-2021-04-04} wrote
\ix{Greene, Brian Randolph}
\begin{quotation}
  Quantum Mechanics in a nutshell:
  A particle goes from here to there
  by sampling every possible trajectory from here to there.

  \[
    \langle x_f,t_f \vert x,t_{\mathit i} \rangle
    =
    \sum_{\text p \in \text{paths}} e^{\mathit iS(\text p) \si{\planckbar}}
  \]
\end{quotation}
\end{VerbatimOut}

\MyIO


%  https://tex.stackexchange.com/questions/96568/how-can-i-align-multiple-cases-environment-simultaneously
\begin{VerbatimOut}{z.out}
\subsection{Question in String Theory / Mass of States / Number Operator}


\textcite{yourlazyphysicist2017} wrote
``I have the following definition of the space-time coordinates'':

\newcommand{\fpt}{{4\pi T}}
\newcommand{\oh}{\frac12}
\newcommand{\snnz}{\sum_{n\ne0}}
\newcommand{\tms}{\tau - \sigma}
\newcommand{\tps}{\tau + \sigma}
\begin{align}
    \text{closed string: }&
        \begin{cases}
            \displaystyle
            X^\mu_R
                = \oh x^\mu
                + \frac1\fpt (\tms) p^\mu
                + \frac i{\sqrt\fpt} \snnz \frac1n \alpha^\mu_n e^{-in(\tms)},\\
            \displaystyle
            X^\mu_L
                = \oh x^\mu
                + \frac1\fpt (\tps) p^\mu
                + \frac i{\sqrt\fpt} \snnz \frac1n \tilde\alpha^\mu_n e^{-in(\tps)}.
        \end{cases}\\[6pt]
    \text{open string: }&
        \begin{cases}
            \displaystyle
            X^\mu_N
                = x^\mu
                + \frac1{\pi T}p^\mu\tau
                + \frac i{\sqrt{\pi T}} \snnz \frac1n \alpha^\mu_n e^{-in\tau} \cos(n\sigma),\\
            \displaystyle
            X^\mu_D
                = x^\mu
                + \frac i{\sqrt{\pi T}} \snnz \frac1n \alpha^\mu_n e^{-in\tau} \sin(n\sigma).
        \end{cases}
\end{align}
\end{VerbatimOut}

\MyIO



% https://www.google.com/url?sa=i&rct=j&q=&esrc=s&source=images&cd=&cad=rja&uact=8&ved=0ahUKEwiSzf370-jmAhXIGs0KHRHyAZQQMwiCASgNMA0&url=https%3A%2F%2Fwww.chegg.com%2Fhomework-help%2Fquestions-and-answers%2Fequations-displacement-atoms-along-linear-chain-d2u-u-m-mass-atoms-c-force-constant-neares-q26052186&psig=AOvVaw1eYq-Q0El0Tbjgbp_Lu2Vv&ust=1578183004388936&ictx=3&uact=3

% M\frac{d^2\mu_n}{dt^2} = C(u_{n_1} - 2u_n + u_{n-1}).

% a^{b} same as a^b     c^{de} f^{g^h} ij^{kl}^{mn}

% superscripts
% subscripts

% operators

%\sum
%\prod

%\alpha
%\beta
%\gamma
%\delta
%\epsilor
%\varepsilon
%\zero
%\eta
%\theta
%\vartheta
%\iota
%\kappa
%\lambda
%\mu
%\nu\xi
%\varrho
%\sigma
%\varsigma
%\tau
%\upsilan
%\pha
%\varphi
%\chi
%\psi
%\omega

%\Gamma
%\Delta
%\Theta
%\Lambda
%\Xi
%\Pi
%\Sigmo
%\Upsilan
%\Phi
%\Psi
%\Omega

%mixed greek and text

%x_min, x_max

%\ldots

%\to

%1 + \frac14 + \frac19 + \cdots = \frac\pi6

%fractions

% frac{\ln x}{\ln\alpha} = log_\alpha x

% \sum_{i=1}^n = 1 + 2 + \cdots + n = \frac{n(n+1)}{2}


% xxxx     \end{verbatim}
% xxxx % Requires \usepackage{amsmath}; use align* for no equation number.
% xxxx \begin{align}
% xxxx   a = {}& b + c\\
% xxxx   x = {}& y + z
% xxxx \end{align}
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx \[
% xxxx   Z =
% xxxx     \left(
% xxxx       \begin{array}{cc}
% xxxx         a& b\\
% xxxx         c& d
% xxxx       \end{array}
% xxxx     \right)
% xxxx \]
% xxxx     \end{verbatim}
% xxxx \[
% xxxx   Z =
% xxxx     \left(
% xxxx       \begin{array}{cc}
% xxxx         a& b\\
% xxxx         c& d
% xxxx       \end{array}
% xxxx     \right)
% xxxx \]
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx \begin{equation}
% xxxx   \begin{split}
% xxxx     a = {}& b + c\\
% xxxx       & {} + d + e
% xxxx   \end{split}
% xxxx \end{equation}
% xxxx     \end{verbatim}
% xxxx \begin{equation}
% xxxx   \begin{split}
% xxxx     a = {}& b + c\\
% xxxx       & {} + d + e
% xxxx     \end{split}
% xxxx \end{equation}
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx \[
% xxxx   (\cos x)^2 + (\sin x)^2 = 1
% xxxx \]
% xxxx     \end{verbatim}
% xxxx \[
% xxxx   (\cos x)^2 + (\sin x)^2 = 1
% xxxx \]
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx     \begin{verbatim}
% xxxx If $X = \cos x$ and $Y = \sin x$ then $X^2 + Y^2 = 1$.
% xxxx     \end{verbatim}
% xxxx If $X = \cos x$ and $Y = \sin x$ then $X^2 + Y^2 = 1$.
% xxxx     \vskip\baselineskip
% xxxx     \hrule
% xxxx     \vskip0.5\baselineskip
% xxxx     \filbreak
% xxxx
% xxxx


==> others/ap-numbers-and-units.tex <==
\ProvidesFile{ap-numbers-and-units.tex}[2021-08-23 numbers and units appendix]

%  Primary sources:
%      See https://www.bipm.org/utils/common/pdf/si-brochure/SI-Brochure-9-EN.pdf.
%      See https://www.nist.gov/pml/special-publication-811/nist-guide-si-chapter-4-two-classes-si-units-and-si-prefixes.
%
%  Notes:
%      See https://www.iso.org/standard/60241.html.

% Historic Vote Ties Kilogram and Other Units to Natural Constants
% NIST
% https://www.nist.gov/news-events/news/2018/11/historic-vote-ties-kilogram-and-other-units-natural-constants
% created 2018-11-16
% updated 2018-12-21
% last retrieved 2018-12-22

% https://www.bipm.org/utils/common/pdf/CGPM-2018/26th-CGPM-Resolutions.pdf
% Resolutions adopted
% 26^e CGPM
% Versailes
% 13--16 November 2018
% last retrieved 2018-12-30

% author Joseph Wright
% date 2018-05-17
% retrieved 2018-12-29
% url ftp://ftp.dante.de/tex-archive/macros/latex/exptl/siunitx/siunitx.pdf


\begin{VerbatimOut}{z.out}
\chapter{NUMBERS AND UNITS}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

Note to self: scientific prefixes, scientific suffixes, tables.

The puthesis 2.0 and after documentclass uses the siunitx
package with some extra definitions in the puthesis.cls
file to do numbers and units.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{Number Examples}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\noindent\begin{tabular}{@{}lll@{}}
  \bfseries Input& \bfseries Output& \bfseries Comment\\
  \tabularspace
  \verb+\num{-0.12345}+& \num{-0.12345}& note the small space after the ``3''\\
  \verb+\num{-0.1234}+&
    \num{-0.1234}&
    note no space between the ``3'' and ``4''\\
  \verb+\num{-.123}+& \num{-.123}& the ``0.'' is inserted automatically\\
  \verb+\num{123}+& \num{123}\\
  \verb+\num{1234}+& \num{1234}\\
  \verb+\num{12345}+& \num{12345}& note the small space after the ``2''\\
  \verb+\num{2e4}+& \num{2e4}\\
  \verb+\num{e5}+& \num{e5}\\
  \verb+\num{2.34567e6}+&
    \num{2.34567e6}&
    note the small space after the ``5''\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{Unit Examples}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

See page~\pageref{se:Complete-List-of-Units}
for the complete list
of units defined by \PurdueThesisLogo.

\noindent\begin{tabular}{@{}lll@{}}
  \bfseries Input& \bfseries Output& \bfseries Comment\\
  \tabularspace
  \verb+\si{\kg}+& \si{\kg}& kilogram\\
  \verb+\si{\m}+& \si{\m}& meter\\
  \verb+\si{\kg\per\m\squared}+&
    \si{\kg\per\m\squared}&
    \(= \si{\kg}/\si{\m\squared}\)\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{Combined Number and Unit Examples}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\begin{tabular}{@{}lll@{}}
  \bfseries Input& \bfseries Output& \bfseries Comment\\
  \tabularspace
  \verb+\SI{12}{\kg}+& \SI{12}{\kg}& 12 kilograms\\
  \verb+\SI{34}{\m}+&  \SI{34}{\m}& 34 meters\\
  % The next input line is too wide for the margins
  % so I'm splitting it into pieces.
  \verb+\SI{4.5e3}{\kg\per\m\squared}+&
    \SI{4.5e3}{\kg\per\m\squared}&
    \(= \num{4.5e3}\,\si{\kg}/\si{\m\squared}\)\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

How many seconds are in a non-leap year that does not have any leap seconds?
% I tried several things and couold not get \cancel to work with \per.
% Mark Senn    2019-12-29
\begin{align*}
           \frac{\SI{365}{\cancel\d}}{\si{\y}}
    \times \frac{\SI{24}{\cancel\h}}{\si{\cancel\d}}
    \times \frac{\SI{60}{\cancel\min}}{\si{\cancel\h}}         
    \times \frac{\SI{60}{\s}}{\si{\cancel\min}}         
    % From http://www.emerson.emory.edu/services/latex/latex_119.html
    %     Spacing in Math Mode
    %     In a math environment, LaTeX ignores the spaces you type
    %     and puts in the spacing that it thinks is best. LaTeX formats
    %     mathematics the way it's done in mathematics texts. If you
    %     want different spacing, LaTeX provides the following four
    %     commands for use in math mode:
    %         \; - a thick space
    %         \: - a medium space
    %         \, - a thin space
    %         \! - a negative thin space
    & = \num{31536000}\;\frac{\si{\s}}{\si{\y}}\\
    & = \SI{31536000}{\s\per\y}\\
    & \approx \SI{3e7}{\s\per\y}\\
    & \approx \text{30 million\,}\si{\s\per\y}\\
\end{align*}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{Binary Prefixes}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The \verb+\kibi+ \ldots \verb+\yobi+
commands are defined immediately after the \verb+\usepackage{siunitx}+ command
in the PurdueThesis.cls file.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\newcolumntype{m}{>{$}r<{$}}  % math mode version of "r" column type
\renewcommand{\t}[4]{\(2^{#1}\) bytes is a #2, \(10^{#3}\) bytes is a #4}
\begin{tabular}{@{}mllll@{}}
  \multicolumn{1}{l}{\bfseries Power}&
    \bfseries Prefix&
    \bfseries Symbol&
    \bfseries Command&
    \bfseries Comment\\
  \tabularspace
  10& kibi& \unit{\kibi\nounit}& \verb+\si{\kibi}+& \t{10}{KB}{3}{KiB}\\
  20& mebi& \unit{\mebi\nounit}& \verb+\si{\mebi}+& \t{20}{MB}{6}{MiB}\\
  30& gibi& \unit{\gibi\nounit}& \verb+\si{\gibi}+& \t{30}{GB}{9}{GiB}\\
  40& tebi& \unit{\tebi\nounit}& \verb+\si{\tebi}+& \t{40}{TB}{12}{TiB}\\
  50& pebi& \unit{\pebi\nounit}& \verb+\si{\pebi}+& \t{50}{PB}{15}{PiB}\\
  60& exbi& \unit{\exbi\nounit}& \verb+\si{\exbi}+& \t{60}{EB}{18}{EiB}\\
  70& zebi& \unit{\zebi\nounit}& \verb+\si{\zebi}+& \t{70}{ZB}{21}{ZiB}\\
  80& yobi& \unit{\yobi\nounit}& \verb+\si{\yobi}+& \t{80}{YB}{24}{YiB}\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{Decimal Prefixes}
\end{VerbatimOut}

\MyIO

\begin{VerbatimOut}{z.out}

\newcolumntype{m}{>{$}r<{$}}  % math mode version of "r" column type
\begin{tabular}{@{}mllll@{}}
  \multicolumn{1}{l}{\bfseries Power}&
    \bfseries Prefix&
    \bfseries Symbol&
    \bfseries Command&
    \bfseries Comment\\
  \tabularspace
  -24& yocto& \unit{\yocto\nounit}& \verb+\si{\yocto}+\\
  -21& zepto& \unit{\zepto\nounit}& \verb+\si{\zepto}+\\
  -18& atto&  \unit{\atto\nounit}&  \verb+\si{\atto}+\\
  -15& femto& \unit{\femto\nounit}& \verb+\si{\femto}+\\
  -12& pico&  \unit{\pico\nounit}&  \verb+\si{\pico}+\\
   -9& nano&  \unit{\nano\nounit}&  \verb+\si{\nano}+\\
   -6& micro& \unit{\micro\nounit}& \verb+\si{\micro}+\\
   -3& milli& \unit{\milli\nounit}& \verb+\si{\milla}+\\
   -2& centi& \unit{\centi\nounit}& \verb+\si{\centi}+\\
   -1& deci&  \unit{\deci\nounit}&  \verb+\si{\deci}+\\
    1& deca&  \unit{\deca\nounit}&  \verb+\si{\deca}+\\
    1& deka&  \unit{\deka\nounit}&  \verb+\si{\deka}+& same as \verb+\si{\deca}+\\
    2& hecto& \unit{\hecto\nounit}& \verb+\si{\hecto}+\\
    3& kilo&  \unit{\kilo\nounit}&  \verb+\si{\kilo}+\\
    6& mega&  \unit{\mega\nounit}&  \verb+\si{\mega}+\\
    9& giga&  \unit{\giga\nounit}&  \verb+\si{\giga}+\\
   12& tera&  \unit{\tera\nounit}&  \verb+\si{\tera}+\\
   15& peta&  \unit{\peta\nounit}&  \verb+\si{\peta}+\\
   18& exa&   \unit{\exa\nounit}&   \verb+\si{\exa}+\\
   21& zetta& \unit{\zetta\nounit}& \verb+\si{\zetta}+\\
   24& yotta& \unit{\yotta\nounit}& \verb+\si{\yotta}+\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{SI Units}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

The International System of Units
(SI)
% !!! Doing
% !!!     \include{tipa}
% !!! in thesis.tex so \textprimstress works
% !!! apparently causes problems with math commands.
% !!! Figure out why the following doesn't work later.
% (%
%   SI,
%   abbreviated from the French Syst\`eme International
%   (d\textprimstress unit\'es)%
% )
is the modern form of the metric system.
There are seven SI base units:

\hspace{40pt}
\begin{tabular}{@{}lll@{}}
  \tabularspace
  \bfseries Name& \bfseries Unit Of&         \bfseries Symbol\\
  \tabularspace
  ampere&         electrical current&        \si{\ampere}\\
  candela&        luminous intensity&        \si{\candela}\\
  kelvin&         thermodynamic temperature& \si{\kelvin}\\
  kg&             mass&                      \si{\kilogram}\\
  meter&          length&                    \si{\meter}\\
  mole&           amount of substance&       \si{\mole}\\
  second&         time&                      \si{\second}\\
\end{tabular}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\section{Complete List of Units}
\label{se:Complete-List-of-Units}
\end{VerbatimOut}

\MyIO

\begin{VerbatimOut}{z.out}

{%
  \ZZbaselinestretch{1}
  \newcommand\vsp{\noalign{\vspace*{6pt}}}
  % From
  % https://tex.stackexchange.com/questions/31508/flushleft-with-p-option-in-tabular
  %     It's necessary to use the \arraybackslash in the last column,
  %     otherwise \\ would not end the table row.  You can use \newline
  %     to end lines in the last column cells (and the regular \\ in
  %     the other column cells).
  %     ...
  %     If you need it often, consider defining a new column type using
  %     array features, as I did here:
  %         \newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
  \newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}%
% \begin{longtable}{@{}P{1.4in}P{1in}llP{1.8in}@{}}
% \begin{longtable}{@{}P{1in}P{1in}llP{1.8in}@{}}
% \begin{longtable}{@{}P{1.2in}P{1in}llP{1.8in}@{}}
% \begin{longtable}{@{}P{90.72pt}P{1in}llP{1.8in}@{}}  % 1.2in (86.72pt) + 4pt = 90.72pt
  \begin{longtable}{@{}P{1.4in}P{1in}llP{1.8in}@{}}% 1.2in (86.72pt) + 4pt = 90.72pt
      \caption{Units and Corresponding Symbols}\\
      \bfseries Name&
        \bfseries Unit Of&
        \bfseries Symbol&
        \bfseries Command&
        \bfseries Is equal to\\
      \vsp
    \endfirsthead
      \caption[]{~\emph{continued}}\\
      \bfseries Name&
        \bfseries Unit Of&
        \bfseries Symbol&
        \bfseries Command&
        \bfseries Is equal to\\
      \vsp
    \endhead
      \vsp
      % I don't know why the \hspace*{-7.5mm} was
      % needed to center this horizontally.
      \multicolumn{5}{@{}c@{}}{\hspace*{-7.5mm}\emph{continued on next page}}%
    \endfoot    
    \endlastfoot
    ampere&
      electrical current&
      \si{\A}&
      \verb+\si{\A}+&
      (SI base unit)\\
    \quad picoampere&
      \ditto&
      \si{\pA}&
      \verb+\si{\pA}+&
      \SI{e-12}{\A}\\ 
    \quad nanoampere&
      \ditto&
      \si{\nA}&
      \verb+\si{\nA}+&
      \SI{e-9}{\A}\\
    \quad microampere&
      \ditto&
      \si{\uA}&
      \verb+\si{\uA}+&
      \SI{e-6}{\A}\\
    \quad milliampere&
      \ditto&
      \si{\mA}&
      \verb+\si{\mA}+&
      \SI{e-3}{\A}\\
    \quad kiloampere&
      \ditto&
      \si{\kA}&
      \verb+\si{\kA}+&
      \SI{e3}{\A}\\
    \vsp
    % \aa ngstr\"om&
    %   length&
    %   \si{\AA}&
    %   \verb+\si{\AA}+&
    %   \SI{e-10}{\m}\\
    \vsp
    arcminute&
      plane angle&
      \si{\arcmin}&
      \verb+\si{\arcmin}+&
      % Changed
      %     \SI{1/60}{\degree}\\
      % to
      1/60\unit{\degree\nounit}\\
    arcsecond&
      plane angle&
      \si{\arcsec}&
      \verb+\si{\arcsec}+&
      % Changed
      %     \SI{1/60}{\arcmin}\\
      % to
      1/60\unit{\arcmin\nounit}\\
    \vsp
    astronomical unit&
      length&
      \si{\au}&
      \verb+\si{\au}+&
      mean earth to\newline sun distance\\
    \vsp
    % From
    %     siunitx - A comprehensive (SI) units package
    %     Joseph Wright
    %     Released 2021-08-04
    %     (this describes v3.0.24, last revised 2021-08-04)
    %     https://mirror.las.iastate.edu/tex-archive/macros/latex/contrib/siunitx/siunitx.pdf
    % page 51:
    %     ...the unit \atomicmassunit has similar deprecated status:
    %     this was listed as with experimentally-determined units
    %     in the 8th Edition of the si Brochure but is equivalent
    %     to the dalton, a unit which remains accepted.
    % atomic mass unit&
    %   mass&
    %   \si{\amu}&
    %   \verb+\si{\amu}+&
    %   \(1/12\) mass of\newline carbon-12 atom\\
    % \vsp
    bar&
      pressure&
      \si{\bar}&
      \verb+\si{\bar}+&
      \SI{e-5}{\Pa}\\
    \quad millibar&
      \ditto&
      \si{\mbar}&
      \verb+\si{\mbar}+&
      \SI{e-3}{\bar}\\
    \vsp
    barn&
      area&
      \si{\b}&
      \verb+\si{\b}+&
      \SI{e-28}{\m\squared}\\
    \vsp
    becquerel&
      radioactivity&
      \si{\Bq}&
      \verb+\si{\Bq}+&
      one radioactive\newline decay per second\\
    \vsp
    bel&
      sound intensity&
      \si{\B}&
      \verb+\si{\B}+&
      10 decibels\\
    \quad decibel&
      \ditto&
      \si{\dB}&
      \verb+\si{\dB}+&
      \SI{e-1}{\B}\\
    \vsp
    bohr&
      length&
      \si{\bohr}&
      \verb+\si{\bohr}+&
      distance between\newline nucleus and electron\newline in hydrogen atom\\
    \vsp
    bushel&
      quantity&
      \si{\bu}&
      \verb+\si{\bu}+&
      see \cite{wikipedia-bushel}\\
    \vsp
    candela&
      luminous intensity&
      \si{\cd}&
      \verb+\si{\cd}+&
      (SI base unit)\\
    \vsp
    coulomb&
      electrical charge&
      \si{\C}&
      \verb+\si{\C}+&
      \si{\A\per\s}\\
    \vsp
    dalton&
      mass&
      \si{\Da}&
      \verb+\si{\Da}+&
      another name for\newline atomic mass unit\\
    \vsp
    day&
      time&
      \si{\d}&
      \verb+\si{\d}+&
      \SI{86400}{\s}\\
    \vsp
    degree&
      plane angle&
      \si{\degree}&
      \verb+\si{\degree}+&
      1/360 of a cicle\\
    \vsp
    degree Celsius&
      temperature&
      \si{\celsius}&
      \verb+\si{\celsius}+&
      xxx\\
    \vsp
    electron mass&
      mass&
      \si{\em}&
      \verb+\si{\em}+&
      xxx\\
    \vsp
    electronvolt&
      energy&
      \si{\eV}&
      \verb+\si{\eV}+&
      xxx\\
    \quad millielectronvolt&
      \ditto&
      \si{\meV}&
      \verb+\si{meV}+&
      \SI{e-3}{\eV}\\
    \quad kiloelectronvolt&
      \ditto&
      \si{\keV}&
      \verb+\si{keV}+&
      \SI{e3}{\eV}\\
    \quad megaelectronvolt&
      \ditto&
      \si{\MeV}&
      \verb+\si{MeV}+&
      \SI{e6}{\eV}\\
    \quad gigaelectronvolt&
      \ditto&
      \si{\GeV}&
      \verb+\si{\GeV}+&
      \SI{e9}{\eV}\\
    \quad teraelectronvolt&
      \ditto&
      \si{\TeV}&
      \verb+\si{\TeV}+&
      \SI{e12}{\eV}\\
    \vsp
    elementary charge&
      electrical charge&
      \si{\ec}&
      \verb+\si{\ec}+&
      \href{https://en.wikipedia.org/wiki/Elementary_charge}{\SI{\approx 1.6e19}{\C}}\\
    \vsp
    farad&
      electrical capacitance&
      \si{\F}&
      \verb+\si{\F}+&
      \si{\s\tothe{4}\A\squared\per\m\squared\per\kg}\\
    \quad femtofarad&
      \ditto&
      \si{\fF}&
      \verb+\si{\fF}+&
      \SI{e-15}{\F}\\
    \quad picofarad&
      \ditto&
      \si{\pF}&
      \verb+\si{\pF}+&
      \SI{e-12}{\F}\\
    \vsp
    foot&
      length&
      \si{\ft}&
      \verb+\si{\ft}+&
      \SI{0.3048}{\m}\\  % not an SI unit
    \vsp
    % gauss: The gauss, symbol G, sometimes Gs, is the cgs unit of measurement of magnetic flux.
    gray&
      absorbed dose of ionizing radiation&
      \si{\Gy}&
      \verb+\si{\Gy}+&
      \si{\J\per\kg}\\
    \vsp
    hartree&
      energy used in molecular orbital calculations&
      \si{\hartree}&
      \verb+\si{\hartree}+&
      xxx\\
    \vsp
    hectare&
      area&
      \si{\ha}&
      \verb+\si{\ha}+&
      \SI{e4}{\m\squared}\\
    \vsp
    henry&
      electrical inductance&
      \si{\H}&
      \verb+\si{\H}+&
      \si{\kg\m\squared\per\s\squared\per\A\squared}\\
    \vsp
    hertz&
      frequency&
      \si{\Hz}&
      \verb+\si{\Hz}+&
      \si{\per\s}\\
    \quad millihertz&
      \ditto&
      \si{\mHz}&
      \verb+\si{\mHz}+&
      \SI{e-3}{\Hz}\\
    \quad kilohertz&
      \ditto&
      \si{\kHz}&
      \verb+\si{\kHz}+&
      \SI{e3}{\Hz}\\
    \quad megahertz&
      \ditto&
      \si{\MHz}&
      \verb+\si{\MHz}+&
      \SI{e6}{\Hz}\\
    \quad gigahertz&
      \ditto&
      \si{\GHz}&
      \verb+\si{\GHz}+&
      \SI{e9}{\Hz}\\
    \quad terahertz&
      \ditto&
      \si{\THz}&
      \verb+\si{\THz}+&
      \SI{e12}{\Hz}\\
    \vsp
    horsepower&
      power&
      \si{\hp}&
      \verb+\si{\hp}+&
      \SI{\approx 745.7}{\W}, {\bfseries IMPORTANT:\newline
        see \href{https://en.wikipedia.org/wiki/Horsepower#Mechanical_horsepower}{Horsepower}}\\
        % not an SI unit
    \vsp
    hour&
      time&
      \si{\h}&
      \verb+\si{\h}+&
      \SI{3600}{\s}\\
    \vsp
    inch&
      length&
      \si{\in}&
      \verb+\si{\in}+&
      \SI{25.4}{\mm}\\  % not an SI unit
    \vsp
    joule&
      work or energy&
      \si{\J}&
      \verb+\si{\J}+&
      \si{\kg\m\squared\per\s\squared}\\
    \quad microjoule&
      \ditto&
      \si{\uJ}&
      \verb+\si{\uJ}+&
      \SI{e-6}{\J}\\
    \quad millijoule&
      \ditto&
      \si{\mJ}&
      \verb+\si{\mJ}+&
      \SI{e-3}{\J}\\
    \quad kilojoule&
      \ditto&
      \si{\kJ}&
      \verb+\si{\kJ}+&
      \SI{e3}{\J}\\
    \quad megajoule&
      \ditto&
      \si{\MJ}&
      \verb+\si{\MJ}+&
      \SI{e6}{\J}\\
    \vsp
    katal&
      catalytic activity&
      \si{\kat}&
      \verb+\si{\kat}+&
      \si{\mol\per\s}\\
    \vsp
    kelvin&
      thermodynamic temperature&
      \si{\K}&
      \verb+\si{\K}+&
      (SI base unit)\\
    \vsp
    kilogram&
      mass&
      \si{\kg}&
      \verb+\si{\kg}+&
      (SI base unit)\\
    \quad femtogram&
      \ditto&
      \si{\fg}&
      \verb+\si{\fg}+&
      \SI{e-15}{\g}\\
    \quad picogram&
      \ditto&
      \si{\pg}&
      \verb+\si{\pg}+&
      \SI{e-12}{\g}\\
    \quad nanogram&
      \ditto&
      \si{\ng}&
      \verb+\si{\ng}+&
      \SI{e-9}{\g}\\
    \quad microgram&
      \ditto&
      \si{\ug}&
      \verb+\si{\ug}+&
      \SI{e-6}{\g}\\
    \quad milligram&
      \ditto&
      \si{\mg}&
      \verb+\si{\mg}+&
      \SI{e-3}{\g}\\
    \quad gram&
      \ditto&
      \si{\g}&
      \verb+\si{\g}+&
      \SI{e-3}{\kg}\\
    \vsp
    kilowatt hour&
      electrical energy&
      \si{\kWh}&
      \verb+\si{\kWh}+&
      \si{\kW\h}\\
    \vsp
    knot&
      speed&
      \si{\kn}&
      \verb+\si{\kn}+&
      \si{\M\per\h}\\
    \vsp
    liter&
      volume&
      \si{\L}&
      \verb+\si{\L}+&
      \SI{e-3}{m\cubed}\\
    \quad microliter&
      \ditto&
      \si{\uL}&
      \verb+\si{\uL}+&
      \SI{e-6}{\L}\\
    \quad milliliter&
      \ditto&
      \si{\mL}&
      \verb+\si{\mL}+&
      \SI{e-3}{\L}\\
    \quad hectoliter&
      \ditto&
      \si{\hL}&
      \verb+\si{\hL}+&
      \SI{e2}{\L}\\
    \vsp
    lumen&
      luminous flux&
      \si{\lm}&
      \verb+\si{\lm}+&
      \si{\cd\sr}\\
    \vsp
    lux&
      illumination&
      \si{\lx}&
      \verb+\si{\lx}+&
      \si{\lm\per\m\squared}\\
    \vsp
    meter&
      length&
      \si{\m}&
      \verb+\si{\m}+&
      (SI base unit)\\
    \quad picometer&
      \ditto&
      \si{\pm}&
      \verb+\si{\pm}+&
      \SI{e-12}{\m}\\
    \quad nanometer&
      \ditto&
      \si{\nm}&
      \verb+\si{\nm}+&
      \SI{e-9}{\m}\\
    \quad micrometer&
      \ditto&
      \si{\um}&
      \verb+\si{\um}+&
      \SI{e-6}{\m}\\
    \quad millimeter&
      \ditto&
      \si{\mm}&
      \verb+\si{\mm}+&
      \SI{e-3}{\m}\\
    \quad centimeter&
      \ditto&
      \si{\cm}&
      \verb+\si{\cm}+&
      \SI{e-2}{\m}\\
    \quad decimeter&
      \ditto&
      \si{\dm}&
      \verb+\si{\dm}+&
      \SI{e-1}{\m}\\
    \quad kilometer&
      \ditto&
      \si{\km}&
      \verb+\si{\km}+&
      \SI{e3}{\m}\\
    \vsp
    % mile: not an SI unit
    millimeter of mercury&
      pressure&
      \si{\mmHg}&
      \verb+\si{\mmHg}+&
      \href{https://en.wikipedia.org/wiki/Millimetre_of_mercury}{\SI{\approx 133}{\Pa}}\\
    \vsp
    minute&
      time&
      \si{\min}&
      \verb+\si{\min}+&
      \SI{60}{\s}\\
    \vsp
    mole&
      amount of substance&
      \si{\mol}&
      \verb+\si{\mol}+&
      (SI base unit)\\
    \quad femtomole&
      \ditto&
      \si{\fmol}&
      \verb+\si{\fmol}+&
      \SI{e-15}{\mol}\\
    \quad picomole&
      \ditto&
      \si{\pmol}&
      \verb+\si{\pmol}+&
      \SI{e-12}{\mol}\\
    \quad nanomole&
      \ditto&
      \si{\nmol}&
      \verb+\si{\nmol}+&
      \SI{e-9}{\mol}\\
    \quad micromole&
      \ditto&
      \si{\umol}&
      \verb+\si{\umol}+&
      \SI{e-6}{\mol}\\
    \quad millimole&
      \ditto&
      \si{\mmol}&
      \verb+\si{\mmol}+&
      \SI{e-3}{\mol}\\
    \quad kilomole&
      \ditto&
      \si{\kmol}&
      \verb+\si{\kmol}+&
      \SI{e3}{\mol}\\
    \vsp
    nautical mile&
      distance&
      \si{\M}&
      \verb+\si{\M}+&
      \SI{1852}{\m}\\
    \vsp
    neper&
      gain, loss, and relative values&
      \si{\Np}&
      \verb+\si{\Np}+&
      1\\
    \vsp
    newton&
      force&
      \si{\N}&
      \verb+\si{\N}+&
      \si{\kg\m\per\s\squared}\\
    \quad millinewton&
      \ditto&
      \si{\mN}&
      \verb+\si{\mN}+&
      \SI{e-3}{\N}\\
    \quad kilonewton&
      \ditto&
      \si{\kN}&
      \verb+\si{\kN}+&
      \SI{e3}{\N}\\
    \quad meganewton&
      \ditto&
      \si{\MN}&
      \verb+\si{\MN}+&
      \SI{e6}{\N}\\
    \vsp
    ohm&
      electrical resistance&
      \si{\ohm}&
      \verb+\si{\ohm}+&
      \si{\kg\m\squared\per\s\cubed\per\A\squared}\\
    \quad milliohm&
      \ditto&
      \si{\mohm}&
      \verb+\si{\mohm}+&
      \SI{e-3}{ohm}\\
    \quad kiloohm&
      \ditto&
      \si{\kohm}&
      \verb+\si{\kohm}+&
      \SI{e3}{ohm}\\
    \quad megaohm&
      \ditto&
      \si{\Mohm}&
      \verb+\si{\Mohm}+&
      \SI{e6}{ohm}\\
    \vsp
    pascal&
      pressure&
      \si{\Pa}&
      \verb+\si{\Pa}+&
      \si{\kg\per\m\per\s\squared}\\
    \qquad kilopascal&
      \ditto&
      \si{\kPa}&
      \verb+\si{\kPa}+&
      \SI{e3}{\Pa}\\
    \qquad megapascal&
      \ditto&
      \si{\MPa}&
      \verb+\si{\MPa}+&
      \SI{e6}{\Pa}\\
    \qquad gigapascal&
      \ditto&
      \si{\GPa}&
      \verb+\si{\GPa}+&
      \SI{e9}{\Pa}\\
    \vsp
    percent&
      hundredths&
      \si{\percent}&
      \verb+\si{\percent}+&
      \SI{e-2}{}\\
    \vsp
    pound&
      weight&
      \si{\lb}&
      \verb+\si{\lb}+&
      \SI{.45359237}{\kg}\\  % not an SI unit
    \vsp
    radian&
      plane angular measurement&
      \si{\rad}&
      \verb+\si{\rad}+&
      \(180/\pi\) \unit{\degree\nounit}\\
    \vsp
    reduced Planck constant&
      angular momentum&
      \si{\planckbar}&
      \verb+\si{\planckbar}+&
      \(\approx \SI{1.05e-34}{\J\s}\)\\
    \vsp
    second&
      time&
      \si{\s}&
      \verb+\si{\s}+&
      (SI base unit)\\
    \quad attosecond&
      \ditto&
      \si{\as}&
      \verb+\si{\as}+&
      \SI{e-18}{\s}\\
    \quad femtosecond&
      \ditto&
      \si{\fs}&
      \verb+\si{\fs}+&
      \SI{e-15}{\s}\\
    \quad picosecond&
      \ditto&
      \si{\ps}&
      \verb+\si{\ps}+&
      \SI{e-12}{\s}\\
    \quad nanosecond&
      \ditto&
      \si{\ns}&
      \verb+\si{\ns}+&
      \SI{e-9}{\s}\\
    \quad microsecond&
      \ditto&
      \si{\us}&
      \verb+\si{\us}+&
      \SI{e-6}{\s}\\
    \quad millisecond&
      \ditto&
      \si{\ms}&
      \verb+\si{\ms}+&
      \SI{e-3}{\s}\\
    \vsp
    siemens&
      conductance&
      \si{\S}&
      \verb+\si{\S}+&
      \si{\per\kg\per\m\squared\s\cubed\A\squared}\\
    \vsp
    sievert&
      dosage of ionizing radiation&
      \si{\Sv}&
      \verb+\si{\Sv}+&
      \si{\m\squared\per\s\squared}\\
    \vsp
    speed of light&
      speed&
      \si{\clight}&
      \verb+\si{\clight}+&
      \SI{299792458}{\m\per\s}\\
    \vsp
    standard deviation&
      amount of variation&
      \si{\SD}&
      \verb+\si{\SD}+&
      $\displaystyle \sqrt{\frac 1{N-1} \sum_{i=1}^N(x_i-\bar x)^2}$\\
    \vsp
    steradian&
      measure of solid angles&
      \si{\sr}&
      \verb+\si{\sr}+&
      \SI{1}{\m\squared\per\m\squared}\\
    \vsp
    tesla&
      magnetic flux density&
      \si{\T}&
      \verb+\si{\T}+&
      \si{\kg\per\s\squared\per\A}\\
    \vsp
    metric ton&
      mass&
      \si{\t}&
      \verb+\si{\t}+&
      \SI{e3}{\kg}\\
    \vsp
    volt&
      electrical potential difference&
      \si{\V}&
      \verb+\si{\V}+&
      \si{\kg\m\squared\per\s\cubed\per\A}\\
    \quad picovolt&
      \ditto&
      \si{\pV}&
      \verb+\si{\pV}+&
      \SI{e-12}{\V}\\
    \quad nanovolt&
      \ditto&
      \si{\nV}&
      \verb+\si{\nV}+&
      \SI{e-9}{\V}\\
    \quad microvolt&
      \ditto&
      \si{\uV}&
      \verb+\si{\uV}+&
      \SI{e-6}{\V}\\
    \quad millivolt&
      \ditto&
      \si{\mV}&
      \verb+\si{\mV}+&
      \SI{e-3}{\V}\\
    \quad kilovolt&
      \ditto&
      \si{\kV}&
      \verb+\si{\kV}+&
      \SI{e3}{\V}\\
    \vsp
    watt&
      power&
      \si{\W}&
      \verb+\si{\W}+&
      \si{\kg\m\squared\per\s\cubed}\\
    \quad microwatt&
      \ditto&
      \si{\uW}&
      \verb+\si{\uW}+&
      \SI{e-6}{\W}\\
    \quad milliwatt&
      \ditto&
      \si{\mW}&
      \verb+\si{\mW}+&
      \SI{e-3}{\W}\\
    \quad kilowatt&
      \ditto&
      \si{\kW}&
      \verb+\si{\kW}+&
      \SI{e3}{\W}\\
    \quad megawatt&
      \ditto&
      \si{\MW}&
      \verb+\si{\MW}+&
      \SI{e6}{\W}\\
    \quad gigawatt&
      \ditto&
      \si{\GW}&
      \verb+\si{\GW}+&
      \SI{e9}{\W}\\
    \vsp
    weber&
      magnetic flux&
      \si{\Wb}&
      \verb+\si{\Wb}+&
      \si{\kg\m\squared\per\s\squared\per\A}\\
    \vsp
    yard&
      length&
      \si{\yd}&
      \verb+\si{\yd}+&
      \SI{.9144}{\m}\\  % not an SI unit
    \vsp
    year&
      time&
      \si{\y}&
      \verb+\si{\y}+&
      \SI{\approx 365.25}{\d}\\  % not an SI unit
  \end{longtable}
}
\end{VerbatimOut}

\MyIO
\endinput

%   Non-SI units accepted for use with the International System of Units.
%   
%   % From
%   %     https://www.bipm.org/en/publications/si-brochure/section2-2-1.html
%   \begin{tabular}{@{}llll@{}}
%     \bfseries Symbol& \bfseries Command& \bfseries Name& \bfseries Unit of\\
%     m^{-1}& reciprocal meter& wavenumber\\
%     m^2& square meter& area\\
%     m^3& cubic meter& volume\\
%     m/s& meter per second& & speed, velocity\\
%     m/s^2& meter per second squared& acceleration\\
%   \end{tabular}
%   
%   In  addition  to  the  units  themselves,
%   siunitx
%   provides  pre-defined  macros  for  all
%   
%   
%   % xxx needs lots more work above and maybe below
%   
%   \section{angles}
%   
%   \ang{1}
%   \ang{1;2}
%   \ang{1;2;3}
%   \ang{;2}
%   \ang{;;3}
%   -\ang{;2}
%   
%   
%   \ang{10}    \\
%   \ang{12.3}  \\
%   \ang{4,5}   \\
%   \ang{1;2;3} \\
%   \ang{;;1}   \\
%   \ang{+10;;} \
%   
%       degrees
%       degrees,minutes
%       degrees,minutes,seconds
%   
%       \degree
%       \arcminute
%       \arcsecond
%   
%       \SI{3.1415}{\degree}
%   
%       \ang{-0;1;}
%   
%       list
%           \SIlist{10;20}{\meter}
%           \SIlist{10;20;30}{\meter}
%       
%   temperatures
%   
%       \degreeCelsius
%       \celsius
%       
%       range
%           \SIrange{1}{5}{\metre}
%           \SIrange{1}{5}{\milli\metre}
%       
%   
%   numbers
%   
%   123                \num{123}     \\
%   1234               \num{1234}    \\
%   12 345             \num{12345}   \\
%   0.123              \num{0.123}   \\
%   0.1234             \num{0.1234}  \\
%   0.123 45           \num{.12345}  \\
%   3.45 x 10-4        \num{3.45d-4} \\
%   -10^{10}           \num{-e10}
%                      \num{12345.67890}
%                      \num{1+-2i}
%                      \num{.3.45}
%   
%       number list
%           \numlist{10;20}
%           \numlist{10;20;30}
%       
%       number range
%           \numrange{10}{20}
%       \celsius


==> others/ap-physics.tex <==
\ProvidesFile{ap-physics.tex}[2021-08-23 Physics appendix]

\begin{VerbatimOut}{z.out}
\chapter{PHYSICS}
\ix{physics//Physics appendix}

Feynman diagrams\ix{Feynman diagram}
show what happens
when elementary particles collide
\cite{feynman-diagram}.
The Feynman diagrams below are from the
\citetitle{ellis2016} documentation \cite{ellis2016}.
\textbf{%
  You must use \texttt{lualatex} instead
  of \texttt{pdflatex}
  to process documents that use the \texttt{tikz-feynman} package.%
}

The input
in the documentation
is different than here because a different random number generator
is used \cite{menke2019}.
I expect this to be corrected.
In the meantime try replacing \texttt{vertical}
with \texttt{vertical'}
and/or switch some \texttt{fermion}
to \texttt{anti} \texttt{fermion} lines \cite{ellis2017}.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\feynmandiagram [large, vertical'=e to f] {
  a -- [fermion] b -- [photon, momentum=\(k\)] c -- [fermion] d,
  b -- [fermion, momentum'=\(p_{1}\)] e -- [fermion, momentum'=\(p_{2}\)] c,
  e -- [gluon] f,
  h -- [anti fermion] f -- [anti fermion] i,
};
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\feynmandiagram [horizontal=a to b] {
  i1 -- [anti fermion] a -- [anti fermion] i2,
  a -- [photon] b,
  f1 -- [fermion] b -- [fermion] f2,
};
\end{VerbatimOut}

\MyIO


==> others/ap-publications.tex <==
\ProvidesFile{ap-publications.tex}[2021-08-23 publications appendix]

\ZZnonchapter{odd}{PUBLICATION(S)}{y}{0pt}
\ix{publication,publications}
\index{\verb+\begin{publicationa}+@\verb+\begin{publication}+}
\index{\verb+\begin{publications}+}
    
The following is based on information in
\cite{template1,template2,template3}.

\renewcommand{\I}{\hspace*{2\ZZparindent}$\bullet$\hspace*{1.5em}}

In a publication or publications section you can\\
  \I list a single publication\index{publication}\\
  \I include a single publication\index{publications}\\
  \I list multiple publications\\
  \I include multiple publications\\
Use\newline
\hspace*{0.5in}\verb+\begin{publication}+\ldots\verb+\end{publication}+\newline
or\newline
\hspace*{0.5in}\verb+\begin{publications}+\ldots\verb+\end{publications}+\newline
to skip to the next page and put the appropriate heading on the
top of the page.

\vspace*{1.5\baselineskip}

\section*{To List a Single Publication}

\begin{verbatim}
  \begin{publication}
    ...list a single publication here...
    ...IMPROVE THIS LATER to show how to do that...
  \end{publication}
\end{verbatim}


\section*{To Include a Single Publication}

\begin{verbatim}
  \begin{publication}
    ...put a single publication here...
    ...IMPROVE THIS LATER to show how to do that...
  \end{publication}
\end{verbatim}


\section*{To List Multiple Publications}

\begin{verbatim}
  \begin{publications}
    ...list multiple publications here...
    ...IMPROVE THIS LATER to show how to do that...
  \end{publications}
\end{verbatim}


\section*{To Include Multiple Publications}

\begin{verbatim}
  \begin{publications}
    ...put the multiple publications here...
    ...IMPROVE THIS LATER to show how to do that...
  \end{publications}
\end{verbatim}


==> others/ap-resources.tex <==
\ProvidesFile{ap-resources.tex}[2021-08-23 resources appendix]

\begin{VerbatimOut}{z.out}
\chapter{RESOURCES}

From the
IEEE Author Center \cite{ieee-author-center}:
\begin{itemize}
  \item
    The
    IEEE Editorial Style Manual for Authors \cite{ieee-editorial-style-manual-for-authors}
    contains a formal set of editorial guidelines.
  \item
    Editing Mathematics \cite{editing-mathematics}
    illustrates how to do mathematics.
  \item
    The
    IEEE Reference Guide \cite{ieee-reference-guide}
    outlines how to cite references.
\end{itemize}

\end{VerbatimOut}

\MyIO


==> others/ap-tables.tex <==
\ProvidesFile{ap-tables.tex}[2021-08-23 tables appendix]

\begin{VerbatimOut}{z.out}
\chapter{TABLES}
\ix{table}
\end{VerbatimOut}

\MyIO


% \newlength{\ta}
% \newlength{\tb}
% \newlength{\tc}
% 
% \settowidth{\ta}{\vbox{\hbox{Money}\hbox{Market}}}
% \settowidth{\tb}{\vbox{\hbox{Stocks}\hbox{and}\hbox{Bonds}}}
% \settowidth{\tc}{\vbox{\hbox{Money}\hbox{Market}\hbox{and}\hbox{Stocks}}}
% 
% {
%     \renewcommand{\baselinestretch}{1}
%     \begin{table}
%       \caption{%
%         \hfil Allocation of the IRA and Keogh Wealth\hfil\break
%         \mbox{}\hfil for Investors With or Without Brokerage Accounts\hfil
%       }
%       \label{tab:ira}
%       \begin{center}
%         \begin{tabular}%
%           {%
%             |%
%             c%
%             |%
%             >{\centering\hspace{0pt}}m{\the\ta}%  Money Market
%             |%
%             c%                                    Stocks 
%             |%
%             c%                                    Bonds
%             |%
%             c%                                    Diversified
%             |%
%             >{\centering\hspace{0pt}}m{\the\tb}%  Stocks and Bonds
%             |%
%             >{\centering\hspace{0pt}}m{\the\tc}%  Money Market and Stocks
%             |%
%             c%                                    Others
%             |%
%           }
%           \hline
%           IMP&
%             Money Market&
%             Stocks&
%             Bonds&
%             Diversified&
%             Stocks and Bonds&
%             Money Market and Stocks&
%             Others\tabularnewline
%           \hline
%           1& 14.19\%& 57.71\%& 12.21\%& 4.50\%& 7.36\%& 3.04\%& 0.99\%\tabularnewline \hline
%           2& 14.08\%& 58.18\%& 12.32\%& 4.44\%& 7.30\%& 2.80\%& 0.88\%\tabularnewline \hline
%           3 &14.26\%& 58.09\%& 12.27\%& 4.50\%& 7.19\%& 2.75\%& 0.94\%\tabularnewline \hline
%           4 &13.94\%& 58.11\%& 12.14\%& 4.78\%& 7.35\%& 2.68\%& 0.99\%\tabularnewline \hline
%           5 &13.92\%& 58.13\%& 11.93\%& 4.56\%& 7.60\%& 2.98\%& 0.88\%\tabularnewline \hline
%         \end{tabular}
%       \end{center}
%       This table presents the allocations of the wealth in the IRA
%       and Keogh accounts in various asset classes.
%       Results from each set of imputed data are presented here.
%       The first column lists the number of the imputations,
%       and rest of the columns lists various allocations.
%       Entrees under each asset class show the percentage of investors
%       who have most of their IRA
%       and Keogh wealth invested in that particular asset class.
%       The asset class Diversified
%       includes stocks,
%       bonds,
%       and money market investments.
%       The asset class Others
%       include investments in various life insurance products,
%       annuities,
%       real estate, etc.
%       \medskip
%     \footnotesize SOURCE: Survey of Consumer Finances,
%     2001,
%     Federal Reserve Board,
%     USA.\par
%   \end{table}
% }


\begin{VerbatimOut}{z.out}

Here is a really simple table.
I was greatly influenced by Herbert Voss' following ideas on typsetting tables \cite{voss2011}:
Use |\toprule|, |\midrule|, and |\bottomrule|.
\index{\verb+\toprule+}
\index{\verb+\midrule+}
\index{\verb+\bottomrule+}
Don't have blank horizontal space to left or right of body of table.
\ix{Voss, Herbert}

% "h" means put table "here"---don't let it float to top or bottom of page
\begin{table}[ht]
  \caption{The first three American Presidents.}
  \vspace*{6pt}
  \centering
    % Table format:
    %     WHAT    DESCRIPTION
    %     @{}     don't put extra space before first column
    %     r       right justify first column
    %     l       left justify second column
    %     @{}     don't put extra space after second column
    \begin{tabular}{@{}rl@{}}
      \toprule
      \bf Number& \bf Name\\
      \midrule
      1& George Washington\\
      2& John Adams\\
      3& Thomas Jefferson\\
      \bottomrule
    \end{tabular}
  \label{ta:first-three-american-presidents}
\end{table}
\ix{table}
\index{\verb+\begin{table}+}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\newpage

Here is the same table with a longer caption.

% "h" means put table "here"---don't let it float to top or bottom of page
\begin{table}[ht]
  \caption{%
    The first three American Presidents.
    This caption is
    much, much, much, much, much, much,
    much, much, much, much, much, much
    longer.%
  }
  \vspace*{6pt}
  \centering
    % Table format:
    %     WHAT    DESCRIPTION
    %     @{}     don't put extra space before first column
    %     r       right justify first column
    %     l       left justify second column
    %     @{}     don't put extra space after second column
    \begin{tabular}{@{}rl@{}}
      \toprule
      \bf Number& \bf Name\\
      \midrule
      1& George Washington\\
      2& John Adams\\
      3& Thomas Jefferson\\
      \bottomrule
    \end{tabular}
  \label{ta:first-three-american-presidents-longer-caption}
\end{table}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\newpage

\LaTeX\ can print horizontal
and vertical rules in tables.
I don't like the way this looks 
and suggest you do not use tables
with lots of horizontal and vertical lines.
\begin{table}[ht]
  \caption{The first three American Presidents with horizontal and vertical lines}
  \vspace*{6pt}
  \centering
    % Table format:
    %     WHAT    DESCRIPTION
    %     @{}     don't put any space left of first column
    %     |       print a vertical rule
    %     c       center column 
    %     |       print a vertical rule
    %     l       left justify column
    %     |       print a vertical rule
    %     @{}     don't put any space right of last column
    \begin{tabular}{@{}|c|l|@{}}
      % "\hline" prints a horizontal rule
      \hline
      \bf \#& \bf Name\\
      \hline
      1& George Washington\\
      \hline
      2& John Adams\\
      \hline
      3& Thomas Jefferson\\
      \hline
    \end{tabular}
  \label{ta:American-Presidents-with-horizontal}
\end{table}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\newpage

Here is a more complicated table.

{
  \UndefineShortVerb{\|}
\begin{table}[ht]
  \caption{C Bitwise Operators}
  \vspace*{6pt}
  \centering
    % Table format:
    %     WHAT    DESCRIPTION
    %     @{}     don't put extra space before first column
    %     c       first column is centered
    %     c       second column is centered
    %     c       third column is centered
    %     c       fourth column is centered
    %     @{}     don't put extra space after fourth column
    \begin{tabular}{@{}cccc@{}}
      \toprule
      \bf A& \bf B& \bf A\(|\)B& \bf A\&B\\[2pt]
      \midrule
      0& 0& 0& 0\\
      0& 1& 1& 0\\
      1& 0& 1& 0\\
      1& 1& 1& 1\\
      \bottomrule
    \end{tabular}
  \label{ta:C-Bitwise}
\end{table}
}
\end{VerbatimOut}

\MyIO


% Plain Tex's \halign command can be used to make tables but it is not
% worth telling users about.  LaTeX is more convenient to make tables
% with generally.
% 
% \begin{VerbatimOut}{z.out}
% 
% You can use Plain \TeX's \verb+\halign+ command to make tables also.
% If you can't do a complicated table using \LaTeX\ commands
% you may want to try using Plain \TeX\ commands.
% \LaTeX's table making commands use Plain \TeX\ commands.
% 
% \begin{table}[ht]
%   \caption{American Presidents using {\tt\char'134 halign}}
%   \hbox to \textwidth{\hss\vbox{\halign{%
%     \strut #&      % 0. \strut
%     \hfil#\qquad&  % 1. Number
%     #\hfil\cr      % 2. Name
%     %
%     & \bf Number& \bf Name\cr
%     & 1& George Washington\cr
%     & 2& John Adams\cr
%     & 3& Thomas Jefferson\cr
%   }}\hss}
%   \label{ta:American-Presidents-using}
% \end{table}
% \end{VerbatimOut}
% 
% \MyIO


\begin{VerbatimOut}{z.out}
\begin{table}[ht]
  \caption{Participant descriptors for twelve practitioners engaged in co-creation activities}
  \label{tab:22participants}
  \center
  \begin{tabular}{@{}cllS@{}}
    \toprule
    \multicolumn{1}{@{}l}{\textbf{Pseudonym}}&
      \textbf{Disciplinary Role}&
      \textbf{Company Type}&
      \multicolumn{1}{l@{}}{\textbf{\# Years of Experience}}\\
    \midrule
    \multicolumn{4}{@{}l@{}}%
    {%
      \textbf{Sequence 1:} $\text{A1.1}\to\text{B2.1}$:
      Overlapping dilemma cards to strengthen and represent%
    }\\
    \multicolumn{4}{@{}l}{ethical complexity
      through practitioner's current ecological complexity model}\\
    1P1& UX Designer& Enterprise (B2C)& 1.5\\
    1P2& Product Manager& Enterprise (B2B)& 5\\
    1P3& Data Scientist& Agency or Consultancy& 1\\
    \noalign{\vspace{8pt}}
    \multicolumn{4}{@{}l@{}}%
    {%
      \textbf{Sequence 2:} $\text{B2.1}\to\text{A1.1}$:
      Building and tracing complexity based on Dilemmas Cards%
    }\\
    \multicolumn{4}{@{}l}{to reconstruct and reflect on their experience}\\
    2P1& UX Designer& Agency or Consultancy& 8\\
    2P2& Product Manager& Agency or Consultancy& 2\\
    2P3& Software Engineer& Enterprise (B2B)& 2\\
    \bottomrule
  \end{tabular}
\end{table}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

\newpage

Here is a table that is too long to fit on one page.

% This is very loosely based on page 106 of _A Guide to LaTeX_, third edition,
% by Helmut Kopka and Patrick W. Daly.
\begin{longtable}{@{}ll@{}}
    \caption{State Abbreviations}\\
    \toprule
    \bf State& \bf Abbreviation\\
    \hline
  \endfirsthead
    \caption[]{\emph{continued}}\\
    \midrule
    \bf State& \bf Abbreviation\\
    \midrule
  \endhead
    \hline
    \multicolumn{2}{r}{\emph{continued on next page}}
  \endfoot
    \bottomrule
  \endlastfoot
  Alabama& AL\\
  Alaska& AK\\
  American Samoa& AS\\
  Arizona& AZ\\
  Arkansas& AR\\
  Armed Forces Europe& AE\\
  Armed Forces Pacific& AP\\
  Armed Forces the Americas& AA\\
  California& CA\\
  Colorado& CO\\
  Connecticut& CT\\
  Delaware& DE\\
  District of Columbia& DC\\
  Federated States of Micronesia& FM\\
  Florida& FL\\
  Georgia& GA\\
  Guam& GU\\
  Hawaii& HI\\
  Idaho& ID\\
  Illinois& IL\\
  Indiana& IN\\
  Iowa& IA\\
  Kansas& KS\\
  Kentucky& KY\\
  Louisiana& LA\\
  Maine& ME\\
  Marshall Islands& MH\\
  Maryland& MD\\
  Massachusetts& MA\\
  Michigan& MI\\
  Minnesota& MN\\
  Mississippi& MS\\
  Missouri& MO\\
  Montana& MT\\
  Nebraska& NE\\
  Nevada& NV\\
  New Hampshire& NH\\
  New Jersey& NJ\\
  New Mexico& NM\\
  New York& NY\\
  North Carolina& NC\\
  North Dakota& ND\\
  Northern Mariana Islands& MP\\
  Ohio& OH\\
  Oklahoma& OK\\
  Oregon& OR\\
  Pennsylvania& PA\\
  Puerto Rico& PR\\
  Rhode Island& RI\\
  South Carolina& SC\\
  South Dakota& SD\\
  Tennessee& TN\\
  Texas& TX\\
  Utah& UT\\
  Vermont& VT\\
  Virgin Islands& VI\\
  Virginia& VA\\
  Washington& WA\\
  West Virginia& WV\\
  Wisconsin& WI\\
  Wyoming& WY\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
  \multicolumn{2}{c}{make this three pages long}\\
\end{longtable}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}

% The table is on the next page.

\newpage

% Set \LTcapwidth (the longtable caption width)
% to \textwidth minus 4 paragraph indent widths.
\setlength{\LTcapwidth}{\textwidth}
\addtolength{\LTcapwidth}{-4\parindent}

\newlength{\twidth}
\newlength{\theight}

\setlength{\twidth}{\textwidth}
\setlength{\theight}{\textheight}

\begin{sidewaystable}
  % The following two lines compensate for what I think is a bug.
  \setlength{\textwidth}{\theight}
  \setlength{\textheight}{\twidth}
  \caption{Sidewaystable of the first three American Presidents.}
  \vspace*{6pt}
  \centering
    \begin{tabular}{@{}rl@{}}
      \toprule
      \bf Number& \bf Name\\
      \midrule
      1& George Washington\\
      2& John Adams\\
      3& Thomas Jefferson\\
      \bottomrule
    \end{tabular}
\end{sidewaystable}
\end{VerbatimOut}

\MyIO

\begin{VerbatimOut}{z.out}
\begin{sidewaystable}
  % The following two lines compensate for what I think is a bug.
  \setlength{\textwidth}{\theight}
  \setlength{\textheight}{\twidth}
  \caption{Two tables can be placed vertically in a sidewaystable environment.}
  \vspace*{6pt}
  \centering
    \begin{tabular}{@{}rl@{}}
      \toprule
      \bf Number& \bf Name\\
      \midrule
      1& George Washington\\
      2& John Adams\\
      3& Thomas Jefferson\\
      \bottomrule
    \end{tabular}
  \vspace*{2\baselineskip}
  \caption{This is the second table in the sideways environment.}
  \vspace*{6pt}
    \begin{tabular}{@{}rl@{}}
      \toprule
      \bf Number& \bf Name\\
      \midrule
      1& George Washington\\
      2& John Adams\\
      3& Thomas Jefferson\\
      \bottomrule
    \end{tabular}
\end{sidewaystable}
\end{VerbatimOut}

\MyIO


% Plain Tex's \halign command can be used to make tables but it is not
% worth telling users about.  LaTeX is more convenient to make tables
% with generally.
% 
% \begin{VerbatimOut}{z.out}
%
% \begin{sidewaystable}
%   % The following two lines compensate for what I think is a bug.
%   \setlength{\textwidth}{\theight}
%   \setlength{\textheight}{\twidth}
%   \caption{%
%     sidewaystable
%     {\tt\cbackslash halign\copencurly}\ldots{\tt\cclosecurly\/} table%
%   }
%   \hbox to \textwidth{\hss\vbox{\halign{%
%     \strut #&      % 0. \strut
%     \hfil#\qquad&  % 1. Number
%     #\hfil\cr      % 2. Name
%     %
%     & \bf Number& \bf Name\cr
%     \noalign{\vskip 2pt}
%     & 1& George Washington\cr
%     & 2& John Adams\cr
%     & 3& Thomas Jefferson\cr
%   }}\hss}
% \end{sidewaystable}
% \end{VerbatimOut}
%
% \MyIO


\begin{VerbatimOut}{z.out}
\begin{sidewaystable}[ht]%
  % The following two lines compensate for what I think is a bug.
  \setlength{\textwidth}{\theight}%
  \setlength{\textheight}{\twidth}%
  \caption{Live Guitar Open String Testing Data - Pitch (\textit{f\textsubscript{0}})}
  \vspace*{6pt}%
  \label{ta:live-guitar}%
  % Define "Live Guitar Test" column.
  \def\lgt#1{\bf Live Guitar Test #1}
  % Define "Note", "Computed", "Measured", "%", and "Accuracy" column headings.
  \def\note{\bf Note}
  \def\cal{\bf Computed}
  \def\mea{\bf Measured}
  \def\per{\bf \%}
  \def\acc{\bf Accuracy}
  % Define "Name", "f_0 (Hz)", "Error", and "Range (\textcent)" column headings.
  \def\name{\bf Name}
  \def\fsz{\bf \textit{f\textsubscript{0}} (Hz)}
  \def\err{\bf Error}
  \def\ran{\bf Range (\textcent)}
  % Make "!" be an invisible character the width of a digit.
  % (All digits in the normal font are the same width.)
  \catcode`\!=\active    \def!{\hphantom 1}
  \hbox to \textwidth
  {%
    \hss
    % From http://zerocapcable.com/?page_id=225
    %     The units of tuning accuracy are cents. A cent is one hundredth
    %     of a semitone.  Since there are 12 semitones in an octave, there
    %     are 1200 cents in an octave.
    % The default \tabcolsep is 6.0pt.
    \setlength{\tabcolsep}{5pt}%
    \begin{tabular}{@{}cc|ccc|ccc|ccc@{}}
      \hline
      \multicolumn{2}{c|}{ }&
        \multicolumn{3}{c|}{\lgt1}&
        \multicolumn{3}{c|}{\lgt2}&
        \multicolumn{3}{c}{\lgt3}\\
      \cline{3-11}
      \note& \cal& \mea& \per& \acc& \mea& \per& \acc& \mea& \per& \acc\\
      \name& \fsz& \fsz& \err& \ran& \fsz& \err& \ran& \fsz& \err& \ran\\
      \hline
      E\textsubscript 2& !82.407& !82.333& 0.0897& $+2$& !82.616& 0.2538& $+6$& !82.474& 0.0814& $+2$\\
      A\textsubscript 2& 110.000& 110.092& 0.0836& $+2$& 110.092& 0.0836& $+2$& 110.092& 0.0836& $+2$\\
      D\textsubscript 3& 146.832& 146.789& 0.0295& $-2$& 146.789& 0.0295& $-2$& 147.239& 0.2769& $+6$\\
      G\textsubscript 3& 195.998& 196.721& 0.3690& $+8$& 195.918& 0.0407& $+2$& 196.721& 0.3690& $+8$\\
      B\textsubscript 3& 246.942& 247.423& 0.1949& $+4$& 246.517& 0.1720& $-4$& 247.423& 0.1949& $+4$\\
      E\textsubscript 4& 329.628& 331.034& 0.4267& $+8$& 331.034& 0.4267& $+8$& 331.034& 0.4267& $+8$\\
      \hline
      \multicolumn{11}{@{}l}{Thanks to Kathryn Schmidt for donating this table.}\\
    \end{tabular}
    \hss
  }
\end{sidewaystable}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
% Define a control sequence to save typing.
% Let * represent zero or more spaces!
% Method 1: \def\g#1{ requires using \g*{10} for 10.
%           Two shifted characters, { and } are needed.
% Method 2: \def\g#1/{ requires using \g*10/ for 10.
%           One unshifted character, / is needed.
% Method 2 requires less work than Method 1.
\def\g#1/{\includegraphics[scale=0.5]{gr-tally-#1.pdf}}%

% Define a length for use later.
\newlength{\tlen}
\setlength{\tlen}{2\parindent}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\begin{table}[h]%
  \label{ta:first-tally-table}
  \caption
  [%
    First tally table.  Use this method.%
  ]%
  {%
    First tally table.  Use this method.  I think it is the simplest.
  }
  \vspace*{6pt}
  %   Note that tabular* instead of tabular is used below.
  %   The {\textwidth} makes the total width of the table the width
  % of the printed area of the page.
  %   The @{\kern\tlen} puts blank space the width of two paragraph indents
  % before the first column.
  %   The @{extracolsep{\fill}} adds \fill space between all subsequent
  % columns.
  %   The lll left justifies the next three columns.
  % after the column.
  %   The @{\kern\tlen} puts blank space the width of two
  % paragraph indents before the first column.
  \begin{tabular*}{\textwidth}{@{\kern\tlen}@{\extracolsep{\fill}}lll@{\kern\tlen}}%
    \g 01/& \g 02/& \g 03/\\
    \g 04/& \g 05/\\
  \end{tabular*}%
\end{table}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\begin{table}[h]
  \caption{%
    Second tally table.
    Don't use this method.
    The method used in the first tally table
    is easier to understand.%
  }%  
  \vspace*{6pt}
  %   Note that tabularx instead of tabular is used below.
  %   The {\textwidth} makes the total width of the table the width
  % of the printed area on the page.
  %   The @{\kern\tlen} puts blank space the width of two paragraph indents
  % before the first column.
  %   The XX makes the first two columns the same width including the space
  % after the column.
  %   The l left justifies the last column.
  %   The @{\kern\tlen} puts blank space the width of two paragraph indents
  % after the last column.
  \begin{tabularx}{\textwidth}{@{\kern\tlen}XXl@{\kern\tlen}}%
    \g 01/& \g 02/& \g 03/\\
    \g 04/& \g 05/\\
  \end{tabularx}%
\end{table}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
\begin{table}[h!]
  \caption{
    Third tally table.
    Don't use this method.
    The method used in the first tally table
    is easier to understand.%
  }%
  \vspace*{6pt}
  \def\t #1/#2/#3/%
  {%
    \hbox to\textwidth{%
      \kern\tlen \g #1/\hfil \g #2/\hfil \g #3/\kern\tlen
    }%
  }%
  \vbox{
    \t 01/02/03/
    \hbox to\textwidth{%
      \kern\tlen \g 04/\hfil \g 05/\hfil \phantom{\g 05/}\kern\tlen
    }%
    }
  \end{table}
\end{VerbatimOut}

\MyIO
  

\begin{VerbatimOut}{z.out}


% Process all unprocessed floats.
% None of the current floats will be after the \FloatBarrier.
\FloatBarrier
\end{VerbatimOut}

\MyIO





%\newlength{\ta}
%\settowidth{\ta}{\vbox{\hbox{Money}\hbox{Market}}}
%\newlength{\tb}
%\settowidth{\tb}{\vbox{\hbox{Stocks}\hbox{and}\hbox{Bonds}}}
%\newlength{\tc}
%\settowidth{\tc}{\vbox{\hbox{Money}\hbox{Market}\hbox{and}\hbox{Stocks}}}
%
%  {\renewcommand{\baselinestretch}{1}
%\begin{table}
%  \caption{\hfil Allocation of the IRA and Keogh Wealth\hfil\break\mbox{}\hfil for Investors With or Without Brokerage Accounts\hfil}
%  \label{tab:ira}
%  \begin{center}
%    \begin{tabular}%
%      {%
%        |%
%        c%
%        |%
%        >{\centering\hspace{0pt}}m{\the\ta}%  Money Market
%        |%
%        c%                                    Stocks 
%        |%
%        c%                                    Bonds
%        |%
%        c%                                    Diversified
%        |%
%        >{\centering\hspace{0pt}}m{\the\tb}%  Stocks and Bonds
%        |%
%        >{\centering\hspace{0pt}}m{\the\tc}%  Money Market and Stocks
%        |%
%        c%                                    Others
%        |%
%      }
%      \hline
%      IMP&
%        Money Market&
%        Stocks&
%        Bonds&
%        Diversified&
%        Stocks and Bonds&
%        Money Market and Stocks&
%        Others\tabularnewline
%      \hline
%      1& 14.19\%& 57.71\%& 12.21\%& 4.50\%& 7.36\%& 3.04\%& 0.99\%\tabularnewline \hline
%      2& 14.08\%& 58.18\%& 12.32\%& 4.44\%& 7.30\%& 2.80\%& 0.88\%\tabularnewline \hline
%      3 &14.26\%& 58.09\%& 12.27\%& 4.50\%& 7.19\%& 2.75\%& 0.94\%\tabularnewline \hline
%      4 &13.94\%& 58.11\%& 12.14\%& 4.78\%& 7.35\%& 2.68\%& 0.99\%\tabularnewline \hline
%      5 &13.92\%& 58.13\%& 11.93\%& 4.56\%& 7.60\%& 2.98\%& 0.88\%\tabularnewline \hline
%    \end{tabular}
%  \end{center}
%  This table presents the allocations of the wealth in the IRA
%  and Keogh accounts in various asset classes.
%  Results from each set of imputed data are presented here.
%  The first column lists the number of the imputations,
%  and rest of the columns lists various allocations.
%  Entrees under each asset class show the percentage of investors
%  who have most of their IRA
%  and Keogh wealth invested in that particular asset class.
%  The asset class Diversified
%  includes stocks,
%  bonds,
%  and money market investments.
%  The asset class Others
%  include investments in various life insurance products,
%  annuities,
%  real estate, etc.
%  \medskip
%  \footnotesize SOURCE: Survey of Consumer Finances,
%  2001,
%  Federal Reserve Board,
%  USA.\par
%\end{table}
%  }


==> others/ap-testing.tex <==
\ProvidesFile{ch-testing.tex}[2021-08-23 testing appendix]

\chapter{TESTING (THIS APPENDIX IS USED FOR TESTING, DOES THIS
  VERY, VERY, VERY, VERY, VERY, VERY, VERY,
  VERY, VERY, VERY, VERY, VERY, VERY, VERY,
  LONG TITLE LOOK OK?)}

\ix{Testing chapter}

\METAPOSTLogo


% {
%   \makeatletter
%     \renewcommand\@makechapterhead[1]%
%     {{%
%       \renewcommand{\baselinestretch}{1} \reset@font
%       \large\bf\thechapter. #1\endgraf
%     }}
% 
%     \chapter{TEST CHAPTER---THIS IS A VERY, VERY, VERY, VERY, VERY, VERY, VERY, VERY, VERY, VERY LONG CHAPTER NAME}
%   \makeatother
% }

\vspace*{0.2in}
\begin{tabular}{@{}lll@{}}
  \bfseries Input&         \bfseries Output&   Comment\\
  \verb+PurdueThesis+&      PurdueThesis&                 just ordinary text\\
  \verb+\PurdueThesisLogo+& \PurdueThesisLogo& PurdueThesis logo, less space between\\
    & & P and u, e and T, and T and h\\
  \verb+\PuThLogo+&         \PuThLogo&         PuTh abbreviation logo\\
\end{tabular}
\vspace*{0.2in}

\ix{%
  alpha//beta//gamma//delta//epsilon//zeta//%
  eta//theta//iota//kappa//lambda//mu//%
  nu//xi//omicron//pi//rho//sigma//%
  tau//upsilon//phi//chi//psi//omega%
}

\section{Figure Captions}


\begin{VerbatimOut}{z.out}

\begin{figure}[h]
  This is the figure.
  \caption
  [%
    This is the caption.  This is the caption.  This is the caption.
    This is the caption.  This is the caption.  This is the caption.%
  ]%
  {%
    This is the caption.  This is the caption.  This is the caption.
    This is the caption.  This is the caption.  This is the caption.%
  }
\end{figure}
\end{VerbatimOut}

\MyIO
  

\begin{VerbatimOut}{z.out}


\section{Apostrophes}

Test apostrophes in text mode: f', f'', and f'''.

Test apostrophes in math mode: \(f',\ f'',\text{ and }f'''\).
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Citations}

Do a bunch of citations to make bibliography over 100 items:\\
\cite{t001,t002,t003,t004,t005,t006,t007,t008,t009,t010}\\
\cite{t011,t012,t013,t014,t015,t016,t017,t018,t019,t020}\\
\cite{t021,t022,t023,t024,t025,t026,t027,t028,t029,t030}\\
\cite{t031,t032,t033,t034,t035,t036,t037,t038,t039,t040}\\
\cite{t041,t042,t043,t044,t045,t046,t047,t048,t049,t050}\\
\cite{t051,t052,t053,t054,t055,t056,t057,t058,t059,t060}\\
\cite{t061,t062,t063,t064,t065,t066,t067,t068,t069,t070}\\
\cite{t071,t072,t073,t074,t075,t076,t077,t078,t079,t080}\\
\cite{t081,t082,t083,t084,t085,t086,t087,t088,t089,t090}\\
\cite{t091,t092,t093,t094,t095,t096,t097,t098,t099,t100}.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}


\section{Footnote}

This is a footnote\footnote{This is a footnote.}%
\index{\verb+\footnote+}%
\ix{footnote}
\end{VerbatimOut}

\MyIO


\section{Section heading in {\protect\scshape SmallCaps} font}
\label{section-headings-with-smallcaps-font}

Section headings with \verb+{\protect\scshape SmallCaps}+ don't work.%
\todoerror{Section headings with {\protect\scshape SmallCaps} don't work.}

\mbox{}

\todowarn{Putting this section in a VerbatimOut environment
  caused a ``'! LaTeX Error: Float(s) lost.'' error.}

This does not work:
\begin{verbatim}
\section{Section heading in {\protect\scshape SmallCaps} font}
\end{verbatim}
use
\begin{verbatim}
\section
  [Section heading with {\protect\scshape SmallCaps}]%
  {Section heading with S{\protect\scriptsize MALL}C{\protect\scriptsize APS}}
\end{verbatim}
instead.


\begin{VerbatimOut}{z.out}


\section{To-do notes}

Make a todo comment.%
\todocomment{Some people use ``to-do'',
  but I want to be consistent with command names.}

The Purdue football game is at noon tomorrow.%
\todowarn{Leave at 10:00---the traffic will be terrible.}

\[
  \sum_1^n = 1, 2, \ldots, n - 1
\]%
\todoerror{$n-1$ should be $n$.}
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
Cite a reference with a very, very, very, \ldots long title
\cite{test-long-title}.
\end{VerbatimOut}

\MyIO


\begin{VerbatimOut}{z.out}
Emily Spreen wrote that the following URLs are invisible in the PDF file.

\begin{verbatim}
@misc{gerstenmaier,
  author = {William H. Gerstenmaier},
  title = {{Progress in Defining the Deep Space Gateway and Transport Plan}},
  month = {March},
  year = {2017},
  howpublished = {\url{https://www.nasa.gov/sites/default/files/atoms/files/nss_chart_v23.pdf}},
  organization = {NASA}
}
\end{verbatim}

I suggest using the following
(added a `2' to the key so they'd have separate entries in the references.).
\begin{verbatim}
@misc{gerstenmaier2,
  author = {William H. Gerstenmaier},
  title = {{Progress in Defining the Deep Space Gateway and Transport Plan}},
  date = {2017-03},
  url = {https://www.nasa.gov/sites/default/files/atoms/files/nss_chart_v23.pdf},
  organization = {NASA}
}
\end{verbatim}

See \cite{gerstenmaier} and \cite{gerstenmaier2} in the REFERENCES.
\end{VerbatimOut}


@misc{hambleton,
  key = {Deep Space Gateway},
  title = {{Deep Space Gateway to Open Opportunities for Distant Destinations}},
  note = {Editor: Kathryn Hambleton},
  year = {2018},
  month = {August 24,},
  howpublished = {\url{https://www.nasa.gov/feature/deep-space-gateway-to-open-opportunities-for-distant-destinations}},
  organization = {NASA}
}
              
\MyIO


==> others/ap-video.tex <==
\ProvidesFile{ap-video.tex}[2021-08-23 video appendix]

\begin{VerbatimOut}{z.out}
\chapter{VIDEO}

% The following is based on information in
%     http://ctan.math.washington.edu/tex-archive/macros/latex/contrib/media9/doc/media9.pdf
% with the following details
%     The media9 Package, v1.19
%     Alexander Grahn
%     https://gitlab.com/agrahn/media9
%     29th July 2021
% See section 2 on page 3 of the document for software dependencies.
% Embed a YouTube video.

This video example doesn't work for me using Firefox on Linux.

\includemedia[
  activate  = pageopen,
  flashvars =
  {
    autohide        = 1   % Autohide controlbar.
    &modestbranding = 1   % No YouTube logo in control bar.
    &rel            = 0   % No related videos after end of this video.
    &showinfo       = 0   % No title and other info before start of video.
  },
  height    = 2.25in,     % 9 x 16 aspect ratio
  width     = 4in
]{}{https://www.youtube.com/watch?v=C0DPdy98e4c}
\end{VerbatimOut}

\MyIO


==> others/ap-vita.tex <==
\ProvidesFile{ap-vita.tex}[2021-08-23 vita appendix]

\begin{vita}
\ix{vita}
\index{\verb+\begin{vita}+}
  
[Put a brief autobiographical sketch here.]

\end{vita}


==> others/ch-introduction_bak.tex <==
\ProvidesFile{ch-introduction.tex}[2021-08-23 introduction chapter]

\chapter{INTRODUCTION}


\newcommand{\btheta}{{\boldsymbol \theta}}
\newcommand{\bbeta}{{\boldsymbol \beta}}
\newcommand{\bxi}{{\boldsymbol \xi}}
\newcommand{\bW}{{\boldsymbol W}}
\newcommand{\bZ}{{\boldsymbol Z}}
\def\hE{\mathbb{E}}
\newcommand{\bphi}{{\boldsymbol \phi}}
\def\cE{{\cal E}}


\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}

\let\origtheassumption\theassumption

\edef\oldassumption{\the\numexpr\value{assumption}+1}



\section{Preliminaries}

A standard sampling algorithm is the Langevin diffusion, which is a stochastic differential equation (SDE) as follows:
\begin{equation}
\label{sde_1}
    d \bbeta_t^{(1)} = - \nabla U(\bbeta_t^{(1)}) dt+\sqrt{2\tau_1} d\bW_t^{(1)},
\end{equation}
where $\bbeta_t^{(1)}\in\mathbb{R}^d$, $U:\mathbb{R}^d\rightarrow \mathbb{R}$ is the energy function, $\{\bW_t^{(1)}\}_{t\geq 0}$  is the standard $d$-dimensional Brownian motion, and $\tau_1>0$ is the temperature. 

Under mild growth conditions on $U$, the Langevin diffusion $\{\bbeta_t^{(1)}\}_{t\geq 0}$ converges to the unique invariant Gibbs distribution $\pi_{\tau_1}(\bbeta^{(1)})\propto \exp(-\frac{U(\bbeta^{(1)})}{\tau_1})$, where $\tau_1$ is crucial for the optimization or sampling of the non-convex energy function $U$. On the one hand, a high-temperature $\tau_1$ achieves the exploration effect: the convergence to the flattened Gibbs distribution of the whole domain is greatly facilitated. However, the high-temperature increases the gap between $\E_{\pi_{\tau_1}}\left[U(\bbeta)\right]$ and $\min U(\bbeta)$\cite{Maxim17}, and affects the connectivity of the geometric properties to the global minimum \cite{Yuchen17}. 
On the other hand, a low-temperature $\tau_1$ leads to the exploitation effect: the solutions explore the local geometry rapidly, but they are more likely to get trapped in local optima, leading to a slow convergence in both optimization and sampling. Therefore, the potential of using a fixed temperature is quite limited


A powerful algorithm called replica exchange Langevin diffusion (reLD), also known as parallel tempering Langevin diffusion, has been proposed to accelerate the convergence of SDE as defined in Eq.(\ref{sde_1}).
reLD proposes to simulate a high-temperature particle for exploration and a low-temperature particle for exploitation and allows them to swap simultaneously. Now consider a higher temperature $\tau_2>\tau_1$ with $\bW^{(2)}$ independent of $\bW^{(1)}$, we have:
\begin{equation}
\label{sde_2}
\begin{split}
    d \bbeta^{(1)} &= - \nabla U(\bbeta^{(1)}) dt+\sqrt{2\tau_1} d\bW_t^{(1)}\\
    d \bbeta^{(2)} &= - \nabla U(\bbeta^{(2)}) dt+\sqrt{2\tau_2} d\bW_t^{(2)},\\
\end{split}
\end{equation}
where $\bbeta^{(2)}, \bW^{(2)}_t\in \mathbb{R}^d$. Eq.(\ref{sde_2}) converges to the invariant Gibbs distribution with density 
\begin{equation}
\label{pt_density}
\begin{split}
    \pi(\bbeta^{(1)}, \bbeta^{(2)})\propto e^{-\frac{U(\bbeta^{(1)})}{\tau_1}-\frac{U(\bbeta^{(2)})}{\tau_2}}.
\end{split}
\end{equation}

By allowing the two particles to swap, reLD follows a Markov process compounded with a Poisson jump process. % with rate $2$ \cite{Paul12}. 
When the jump rate is specified as the Metropolis form $S(\bbeta^{(1)}, \bbeta^{(2)}):=e^{ \left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left(U(\bbeta^{(1)})-U(\bbeta^{(2)})\right)}$, the invariant distribution remains the same as  ($\ref{pt_density}$).

 

\section{Replica Exchange Stochastic Gradient Langevin Dynamics}

The wide adoption of the replica exchange Monte Carlo in traditional MCMC algorithms motivates us to design replica exchange stochastic gradient Langevin dynamics for DNNs, but the straightforward extension of reLD to replica exchange stochastic gradient Langevin dynamics is highly non-trivial \cite{Chen14, yian2015, Simsekli2016}. In this section, we will first show that na\"ive extensions of replica exchange Monte Carlo to SGLD (na\"ive reSGLD) don't yield correct MCMC algorithms and lead to large biases. Afterward, we will present an adaptive replica exchange stochastic gradient Langevin dynamics (reSGLD) that will automatically adjust the bias and yield a good approximation to the correct distribution under mild assumptions.  

\subsection{Na\"ive reSGLD}

We denote the entire data by $\mathcal{D}=\{\bm{\mathrm{d}}_i\}_{i=1}^N$, where $\bm{\mathrm{d}}_i$ is a data point. Given the model parameter $\widetilde \bbeta$, the log-likelihood is defined as follows
\begin{equation}
\Pi(\widetilde \bbeta) = \sum_{i=1}^N \log P(\bm{\mathrm{d}}_i\mid\widetilde \bbeta).
\end{equation}
When the number of data points $N$ is large, it is expensive to evaluate $\Pi(\widetilde \bbeta)$ directly. Instead, we propose to approximate the log-likelihood with a mini-batch of data $\mathcal{B}=\{\bm{\mathrm{d}}_{s_i}\}_{i=1}^n$, where $s_i\in \{1, 2, ..., N\}$. We can easily check that if $\mathcal{B}$ is sampled randomly with or without replacement, we obtain the following unbiased estimator of the log-likelihood
\begin{equation}
\widetilde \Pi(\widetilde \bbeta) = \frac{N}{n}\sum_{i=1}^n \log P(\bm{\mathrm{d}}_{s_i}\mid \widetilde \bbeta).
\end{equation}
Consider the negative log-posterior (energy function) $L(\widetilde \bbeta)\propto -\log p(\widetilde \bbeta) - \Pi(\widetilde \bbeta)$, where $p(\widetilde \bbeta)$ is a proper prior, we can easily obtain the unbiased estimator $\widetilde L(\widetilde \bbeta)\propto -\log p(\widetilde \bbeta) -\widetilde \Pi(\widetilde \bbeta)$ for $L(\widetilde \bbeta)$ given a large dataset. To scale up the computations of MCMC in DNNs, SGLD proposes to generate iterates as follows:
\begin{equation}
\begin{split}
&\widetilde \bbeta_{k+1}=\widetilde \bbeta_k - \eta_k \nabla \widetilde{L}(\widetilde \bbeta_k)+\sqrt{2\eta_k\tau_1}\bxi_k,\\
\end{split}
\end{equation}
where $\eta_k$ is the learning rate, the stochastic gradient $\nabla \widetilde{L}(\widetilde \bbeta_k)$ is the unbiased estimator of the exact gradient $\nabla L(\widetilde \bbeta_k)$, $\tau_1>0$ denotes the temperature, $\bxi$ is a standard $d$-dimensional Gaussian vector with mean $\bm{0}$ and identity covariance matrix. It is known that SGLD asymptotically converges to a unique invariant distribution $\pi(\widetilde \bbeta)\propto \exp\left(-L(\widetilde \bbeta)/\tau_1\right)$ \cite{Teh16} as $\eta\rightarrow 0$. If we simply use stochastic gradient in the replica exchange gradient Langevin dynamics, we have
\begin{equation}
\label{naive_resgld}
\begin{split}
    \widetilde \bbeta^{(1)}_{k+1} &= \widetilde \bbeta^{(1)}_{k}- \eta_k^{(1)} \nabla \widetilde L(\widetilde \bbeta^{(1)}_k)+\sqrt{2\eta_k^{(1)}\tau_1} \bxi_k^{(1)}\\
    \widetilde \bbeta^{(2)}_{k+1} &= \widetilde \bbeta^{(2)}_{k} - \eta_k^{(2)}\nabla \widetilde L(\widetilde \bbeta^{(2)}_k)+\sqrt{2\eta_k^{(2)}\tau_2} \bxi_k^{(2)}.\\
\end{split}
\end{equation}
Furthermore, we swap the Markov chains in (\ref{naive_resgld}) with the na\"ive stochastic swapping rate $\mathbb{S}(\widetilde \bbeta^{(1)}, \widetilde \bbeta^{(2)})$:
\begin{equation}
\label{swap_naive}
\begin{split}
    &\mathbb{S}(\widetilde \bbeta^{(1)}, \widetilde \bbeta^{(2)})=e^{ \left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left(\widetilde L(\widetilde \bbeta^{(1)})-\widetilde L(\widetilde \bbeta^{(2)})\right)}.\\
\end{split}
\end{equation}
Apparently, the unbiased estimators $\widetilde L(\widetilde \bbeta^{(1)})$ and $\widetilde L(\widetilde \bbeta^{(2)})$ do not provide an unbiased estimator of the swapping rate $S(\widetilde \bbeta^{(1)}, \widetilde \bbeta^{(2)})$ after exponentiating (\ref{swap_naive}), which leads to a largely-biased sampling algorithm.




\subsection{Replica Exchange Stochastic Gradient Langevin Dynamics with Correction}
A viable MCMC algorithm requires the approximately unbiased estimators \cite{Gyongy86, Amel} of the swapping rates to ``satisfy'' the detailed balance property \cite{penalty_swap99, Geoff12, Matias19}. When we make normality assumption on $\widetilde L(\btheta)\sim\mathcal{N}( L(\btheta), \sigma^2)$, it follows 
\begin{equation}
\label{diff_L}
    \widetilde L(\widetilde \bbeta^{(1)})-\widetilde L(\widetilde \bbeta^{(2)})=
    L(\widetilde \bbeta^{(1)})-L(\widetilde \bbeta^{(2)}) + \sqrt{2}\sigma W_1, \\
\end{equation}
where $W_1$ is a Brownian motion at $t=1$, and follows the standard normal distribution. Consider the geometric Brownian motion of $\{\widetilde S_t\}_{t\in[0,1]}$ in each swap as a Martingale
\begin{equation}
\begin{split}
\label{analytic}
    \widetilde S_t&=e^{\left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left(\widetilde L(\widetilde \bbeta^{(1)})-\widetilde L(\widetilde \bbeta^{(2)})-\sigma^2 t\right)}\\
    &=e^{\left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left(L(\widetilde \bbeta^{(1)})-L(\widetilde \bbeta^{(2)})-\sigma^2 t+\sqrt{2}\sigma W_t\right)}.\\
\end{split}
\end{equation}
Take the derivative of $\widetilde S_t$ with respect to $t$ and $W_t$
\begin{equation}
    \frac{d \widetilde S_t}{d t}=-\sigma^2 \widetilde S_t,\  \frac{d \widetilde S_t}{dW_t}=\sqrt{2}\sigma S_t,\  \frac{d^2 \widetilde S_t}{d W_t^2}=2\sigma^2 \widetilde S_t.
\end{equation}
It\^{o}'s lemma gives, 
\begin{equation*}
\begin{split}
    d \widetilde S_t&=(\frac{d\widetilde S_t}{dt}+\frac{1}{2}\frac{d^2 \widetilde S_t}{dW_t^2})dt + (\frac{d\widetilde S_t}{dW_t})dW_t= \sqrt{2}\sigma \widetilde S_t d W_t.
\end{split}
\end{equation*}
Notice that the above process yields the same expectation for all $t\in [0, 1]$. By fixing $t=1$ in (\ref{analytic}), we have
\begin{equation}
\begin{split}
\label{sto_acceptance}
    \widetilde S_1&=e^{ \left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left( \widetilde L(\widetilde \bbeta^{(1)})- \widetilde L(\widetilde \bbeta^{(2)})-\sigma^2\right)},\\
\end{split}
\end{equation}
where the stochastic swapping rate $\widetilde S_1$ is an unbiased estimator of $\widetilde S_0=e^{\left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left(L(\widetilde \bbeta^{(1)})-L(\widetilde \bbeta^{(2)})\right)}$, and the variance $\sigma^2$ is also viewed as the correction term to reduce the bias from the swaps \cite{penalty_swap99}. 

An advantage of interpreting the correction term from the perspective of geometric Brownian motion is that we can naturally extend it to geometric L\'{e}vy process \cite{David04}, which is more suitable for the heavy-tailed energy noise \cite{Simsekli2019b}. Admittedly, the estimation of the tail-index of extreme-value distributions and the correction under L\'{e}vy process go beyond the scope of this paper, so we leave it for future works.



\subsection{Adaptive Replica Exchange Stochastic Gradient Langevin Dynamics}

In reality, the exact variance (correction) $\sigma^2$ of (\ref{sto_acceptance}) is hardly known and subject to estimation. The normality assumption may be violated and even no longer time-independent.



\subsubsection{Fixed Variance $\sigma^2$}
We use stochastic approximation to adaptively estimate the unknown corrections while sampling from the posterior. In each SA step, we obtain an unbiased sample variance $\tilde \sigma^2$ for the true $\sigma^2$ and update the adaptive estimate $\hat \sigma_{m+1}^2$ through
\begin{equation}
    \hat \sigma^2_{m+1} = (1-\gamma_m)\hat \sigma^2_{m}+\gamma_m \tilde \sigma^2_{m+1},
\end{equation}
where $\gamma_m$ is the smoothing factor at the $m$-th SA step. The SA step is updated less frequently than the standard sampling to reduce the computational cost. When the normality assumption holds, we notice that $\hat \sigma_{m}^2=\sum_{i=1}^m \tilde \sigma_{i}^2/m$ when $\gamma_m=\frac{1}{m}$. Following central limit theorem (CLT), we have that $\hat \sigma_m^2-\sigma^2 =\mathcal{O}(\frac{1}{\sqrt{m}})$. In what follows, the adaptive algorithm forms an inhomogenous Markov chain, which is expected to achieve an \emph{optimization-sampling equilibrium}.   

In practice, the normality assumption is likely to be violated when we use a small batch size $n$, but the unknown distribution asymptotically approximates the normal distribution as $n\rightarrow \infty$ and yield a bias $\mathcal{O}(\frac{1}{n})$ in each SA step. Besides, the mini-batch setting usually introduces a very large noise on the estimator of the energy function, which requires a large correction term and leads to almost-zero swapping rates. To handle this issue, we introduce a correction factor $F$ to reduce the correction term from $\hat \sigma^2$ to $\frac{\hat \sigma^2}{F}$. We note that a large $F>1$ introduces some bias, but may significantly increase the acceleration effect, giving rise to an acceleration-accuracy trade-off in finite time. Now, we show the resulting algorithm in Alg.\ref{alg}.


\begin{algorithm}[tb]
   \caption{Adaptive Replica Exchange Stochastic Gradient Langevin Dynamics Algorithm. The SA (stochastic approximation) step is usually updated less frequently than the sampling step to reduce the cost. In DNN models, a larger smoothing factor $\gamma_m$ tracks the dynamics of time-varying corrections better but is less robust.}
   \label{alg}
\begin{algorithmic}
\REPEAT
   \STATE{\textbf{Sampling Step}}
   \begin{equation*}
       \begin{split}
           \widetilde \bbeta^{(1)}_{k+1} &= \widetilde \bbeta^{(1)}_{k}- \eta_k^{(1)} \nabla \widetilde L(\widetilde \bbeta^{(1)}_k)+\sqrt{2\eta_k^{(1)}\tau_1} \bxi_k^{(1)}\\
    \widetilde \bbeta^{(2)}_{k+1} &= \widetilde \bbeta^{(2)}_{k} - \eta_k^{(2)}\nabla \widetilde L(\widetilde \bbeta^{(2)}_k)+\sqrt{2\eta_k^{(2)}\tau_2} \bxi_k^{(2)},\\
       \end{split}
   \end{equation*}
   \STATE{\textbf{SA Step}}
   \STATE{Obtain an unbiased estimate $\tilde \sigma_{m+1}^2$ for $\sigma^2$.}
   \begin{equation*}
   \begin{split}
       &\hat \sigma^2_{m+1} = (1-\gamma_m)\hat \sigma^2_{m}+\gamma_m \tilde \sigma^2_{m+1},\\
   \end{split}
   \end{equation*}
   \STATE{\textbf{Swapping Step}}
   \STATE{Generate a uniform random number $u\in [0,1]$.}
   \begin{equation*}
       \textstyle \hat S_1=\exp\left( \left(\frac{1}{\tau_1}-\frac{1}{\tau_2}\right)\left( \widetilde L(\widetilde \bbeta^{(1)})- \widetilde L(\widetilde \bbeta^{(2)})-\frac{\hat \sigma^2_{m+1}}{F}\right)\right)
   \end{equation*}
   \IF{$u<\hat S_1$}
   \STATE Swap $\widetilde \bbeta_{k+1}^{(1)}$ and $\bbeta_{k+1}^{(2)}$.
   \ENDIF
   \STATE{Anneal the temperatures $\tau_1$ and $\tau_2$ if appliable.}
   \UNTIL{$k=k_{\max}$}
\end{algorithmic}
\end{algorithm}

\subsubsection{Time-varying Variance $\sigma^2$}
In practice, the variance $\sigma^2$ usually varies with time. For example, in the optimization of residual networks on CIFAR10 and CIFAR100 datasets, we notice from Fig.\ref{cifar_biases}(a-b) that the corrections (variances) are time-varying. As such, we cannot use a fixed correction anymore to deal with the bias. The treatment for the time-varying corrections includes standard methods for time-series data, and a complete recipe for modeling the data goes beyond our scope. We adopt the method of simple exponential smoothing due to its simplicity and robustness \cite{Gardner06}, and the algorithm is still an adaptive sampling algorithm, which resembles the stochastic approximation with a fixed learning rate $\alpha$ so that
\begin{equation}
\label{smoothing}
    \hat \sigma^2_{m+1} = (1-\alpha)\hat \sigma^2_{m}+\alpha \tilde \sigma^2_{m+1},
\end{equation}
where only one insensitive hyper-parameter $\alpha$ is introduced. 

The exponential smoothing method has been proven optimal for a general class of state-space models 
%with two sources of error 
\cite{muth64} and acts as robust filters to remove high-frequency noise. It can be viewed as a special case of autoregressive integrated moving average (ARIMA) (0,1,1) model but often outperforms the ARIMA equivalents because it is less sensitive to the model selection error \cite{john66}. From the regression perspective, the exponential smoothing can be viewed as a zero-degree
local polynomial kernel model \cite{Gijbels99}, which is robust to distributional assumptions.




\section{Convergence analysis in Wasserstein distance}

We theoretically analyze the acceleration effect and the accuracy of reSGLD in terms of 2-Wasserstein distance between the Borel probability measures $\mu$ and $\nu$ on $\mathbb{R}^d$ 
\begin{equation*}
    \mathcal{W}_2(\mu, \nu):=\inf_{\Gamma\in \text{Couplings}(\mu, \nu)}\sqrt{\int\|\bbeta_{\mu}-\bbeta_{\nu}\|^2 d \Gamma(\bbeta_{\mu}, \bbeta_{\nu})},
\end{equation*}
where $\|\cdot\|$ is the Euclidean norm, and the infimum is taken over all joint distributions $\Gamma(\bbeta_{\mu}, \bbeta_{\nu})$ with $\mu$ and $\nu$ being its marginal distributions.

Our analysis begins with the fact that reSGLD in Algorithm.\ref{alg} tracks the replica exchange Langevin diffusion (\ref{sde_2}) in 2-Wasserstein ($\mathcal{W}_2$) distance. For ease of analysis, we consider a fixed learning rate $\eta$ for both chains. reSGLD can be viewed as a special discretization of the continuous-time Markov jump process. In particular, it differs from the standard discretization of the continuous-time Langevin diffusion \cite{Maxim17,Issei14, chen2018accelerating} in that we need to consider the discretization of the Markov jump process in a stochastic environment. To handle this issue, we follow \cite{Paul12} and view the swaps of positions as swaps of the temperatures, which have been proven equivalent in distribution.
\begin{lemma}[Discretization Error]
\label{th:1}
Given the smoothness and dissipativity assumptions in the appendix, and a small learning rate $\eta$, we have that
\begin{equation*}
    \begin{split}
&    \scriptstyle \hE[\sup_{0\le t\le T}\|\bbeta_t-\widetilde \bbeta^{\eta}_t\|^2] \le \mathcal{\tilde O}(\eta+\max_i\hE[\|\bphi_i\|^2]+ \max_{i}\sqrt{\hE\left[\mid\psi_{i}\mid^2\right]}),\\
    \end{split}
\end{equation*}
where $\widetilde \bbeta^{\eta}_t$ is the continuous-time interpolation for reSGLD, $\bphi:=\nabla \widetilde U-\nabla U$ is the noise in the stochastic gradient, and $\psi:=\widetilde S-S$ is the noise in the stochastic swapping rate. 
\end{lemma}



Then we quantify the evolution of the 2-Wasserstein distance between $\nu_{t}$ and the invariant distribution $\pi$, where $\nu_t$ is the probability measure associated with reLD at time $t$. The key tool is the exponential decay of entropy when $\pi$ satisfies the log-Sobolev inequality (LSI) \cite{Bakry2014}. To justify LSI, we first verify LSI for reLD without swaps, which is a direct result \cite{Cattiaux2010} given the Lyapunov function criterion and the Poincar\'{e} inequality \cite{chen2018accelerating}. Then we verify LSI for reLD with swaps by analyzing the Dirichlet form. Finally, the exponential decay of the 2-Wasserstein distance follows from the Otto-Villani theorem \cite{Bakry2014} by connecting 2-Wasserstein distance with the relative entropy.

\begin{lemma}[Accelerated exponential decay of $\mathcal{W}_2$]\label{exponential decay}
Under the smoothness and dissipativity assumptions, we have that the replica exchange Langevin diffusion converges exponentially fast to the invariant distribution $\pi$:
\begin{equation}
    \mathcal{W}_2(\nu_t,\pi) \leq  \delta_0 e^{-k\eta(1+\delta_S)/c_{\text{LS}}},
\end{equation}
where $\delta_{S}:=\inf_{t>0}\frac{\cE_S(\sqrt{\frac{d\nu_t}{d\pi}})}{\cE(\sqrt{\frac{d\nu_t}{d\pi}})}-1$ is the very \textbf{acceleration effect} depending on the swapping rate $S$, $\cE$ and $\cE_S$ are the Dirichlet forms defined in the appendix, $c_{\text{LS}}$ is the constant in the log-Sobolev inequality, $\delta_0=\sqrt{2c_{\text{LS}}D(\nu_0\|\pi)}$, 
\end{lemma}{}


Finally, combining the definition of Wasserstein distance and the triangle inequality, we have that 

\begin{theorem}[Convergence of reSGLD]Let the smoothness and dissipativity assumptions hold. For the invariant measure $\{\mu_{k}\}_{k\ge 0}$ associated with the discrete dynamics $\{\widetilde \bbeta_k\}_{k\ge 1}$, we have the following estimates, for $k\in \mathbb N^{+}$, 
\begin{equation*}
\begin{split}
    \mathcal{W}_2(\mu_{k}, &\pi) \le  \delta_0 e^{-k\eta(1+\delta_S)/c_{\text{LS}}}+\footnotesize{\mathcal{\tilde O}(\eta^{\frac{1}{2}}+\max_i(\hE[\|\bphi_i\|^2])^{\frac{1}{2}}+ \max_{i}(\hE\left[\mid\psi_{i}\mid^2\right]})^{\frac{1}{4}}),\\
\end{split}
\end{equation*}
where $\delta_0=\sqrt{2c_{\text{LS}}D(\mu_0\|\pi)}$, $\delta_{S}:=\min_{i}\frac{\cE_S(\sqrt{\frac{d\mu_i}{d\pi}})}{\cE(\sqrt{\frac{d\mu_i}{d\pi}})}-1$.
\end{theorem}{}



Ideally, we want to boost the acceleration effect $\delta_S$ by using a larger swapping rate $S$ and increase the accuracy by reducing the mean squared errors $\hE[\|\bphi_i\|^2]$ and $\hE[\mid\psi_i \mid^2]$. One possible way is to apply a large batch size, which may be yet inefficient given a large dataset. Another way is to seek a balance between the acceleration effect and accuracy by tuning the correction factor $F$. In practice, a larger $F$ leads to a larger acceleration effect and also injects more biases.




\section{Experiments}

\subsection{Simulated Scenarios on Multimodal Sampling}

In this group of experiments, we evaluate the acceleration effects and the biases for reSGLD on multi-modal distributions based on different assumptions on the estimators for the energy function. As a comparison, we choose SGLD and the na\"ive reSGLD without corrections as baselines. The learning rates $\eta^{(1)}$ and $\eta^{(2)}$ are both set to 0.03, and the temperatures $\tau_1$ and $\tau_2$ are set to 1 and 10, respectively. In particular, SGLD uses the learning rate $\eta^{(1)}$ and the temperature $\tau_1$. We simulate 100,000 samples from each distribution and propose to estimate the correction every 100 iterations. The correction estimator is calculated based on the variance of 10 samples of $\widetilde U_1(x)$. The initial correction is set to 100 and the step size $\gamma_m$ for stochastic approximation is chosen as $\frac{1}{m}$. The correction factor $F$ is 1 in the first two examples.


We first demonstrate reSGLD on a simple Gaussian mixture distribution $e^{-U_1(x)}\sim 0.4 \mathcal{N}(-3, 0.7^2)+0.6\mathcal{N}(2, 0.5^2)$, where $U_1(x)$ is the energy function. We assume we can only obtain the unbiased energy estimator $\widetilde U_1(x)\sim \mathcal{N}(U_1(x), 2^2)$ and the corresponding stochastic gradient at each iteration.  From Fig.\ref{mixture}(a,b), we see that SGLD suffers from the local trap problem and takes a long time to converge. The na\"ive reSGLD algorithm alleviated the local trap problem, but is still far away from the ground truth distribution without a proper correction. The na\"ive reSGLD converges faster than reSGLD in the early phase due to a higher swapping rate, but ends up with a large bias when the training continues. By contrast, reSGLD successfully identifies the right correction through adaptive estimates and yields a close approximation to the ground truth distribution. The high-temperature chain serves as a bridge to facilitate the movement, and the local trap problem is greatly reduced. 

\begin{figure*}[!ht]
  \centering
  \subfigure[$\scriptstyle \widetilde U_1(x)\sim \mathcal{N}(U_1(x), 2^2)$.]{\includegraphics[scale=0.22]{figures/sim_mixture_1_grey.pdf}}\label{fig: 22a}
  \subfigure[Convergence evaluation.]{\includegraphics[scale=0.22]{figures/decay_rate_grey.pdf}}\label{fig: 22b}
  \subfigure[$\scriptstyle \widetilde U_2(x)\sim U_2(x)+ t(\nu=5)$.]{\includegraphics[scale=0.22]{figures/sim_mixture_2_grey.pdf}}\label{fig: 22c}
  \subfigure[$\scriptstyle \widetilde U_3(x)\sim U_3(x)+7 t(\nu=10)$.]{\includegraphics[scale=0.22]{figures/sim_mixture_3_grey.pdf}}\label{fig: 22d}
  \caption{Evaluation of reSGLD on Gaussian mixture distributions, where reSGLD proposes to use stochastic approximation to estimate the unknown corrections and the na\"ive reSGLD doesn't make any corrections to adjust the swapping rates.}\label{mixture}
  \vspace{-1em}
\end{figure*}


In the second example, we relax the normality assumption to a heavy-tail distribution. Given a Gaussian mixture distribution $e^{-U_2(x)}\sim 0.4 \mathcal{N}(-4, 0.7^2)+0.6\mathcal{N}(3, 0.5^2)$, we assume that we can obtain the stochastic energy estimator $\widetilde U_2(x)\sim U_2(x)+t(\nu=5)$, where $t(\nu=5)$ denotes the Student's t-distribution with degree of freedom 5. We see from Fig.\ref{mixture}(c) that reSGLD still gives a good approximation to the ground true distribution while the others don't.


In the third example, we show a case when the correction factor $F$ is useful. We sample from a Gaussian mixture distribution $e^{-U_3(x)}\sim 0.4 \mathcal{N}(-6, 0.7^2)+0.6\mathcal{N}(4, 0.5^2)$. We note that the two modes are far away from each other and the distribution is more difficult to simulate. More interestingly, we assume $\widetilde U_3(x)\sim U_3(x)+7 t(\nu=10)$, which requires a large correction term and ends up with no swaps in the finite 100,000 iterations at $F=1$. In such a case, the unbiased algorithm behaves like the ordinary SGLD as in Fig.\ref{mixture}(c) and still suffers from the local trap problems. To achieve larger acceleration effects to avoid local traps and maintain accuracy, we try $F$ at $2$, $4$ and $\infty$, where the reSGLD with $F=\infty$ is equivalent to the na\"ive reSGLD. We see from Fig.\ref{mixture}(d) that $F=2$ shows the best approximations, despite that the swapping rate $S$ is only $0.4\%$. Further increases on the acceleration effect via larger correction factors $F$ give larger swapping rates (7.1\% and 46\%) and potentially accelerate the convergence in the beginning. However, the biases become more significant as we increase $F$ and lead to larger errors in the end.

==> packages/ap-music.tex <==
\ProvidesFile{ap-music.tex}[2021-08-23 music appendix]

\begin{VerbatimOut}{z.out}
\chapter{MUSIC}
\ix{music//Music appendix}

To get the following printed music score I did the following steps.
\begin{itemize}
  \item
    Get the ``Example of LilyPond input file''
    from the Wikipedia LilyPond page \cite{wikipedia-lilypond}
    and put it in a \verb+fib.ly+ file.
  \item
    Ran \verb+lilypond fib.ly+ and got the following \verb+fib.pdf+ file:
\end{itemize}
\ix{LilyPond music typesetting software}

\noindent \includegraphics[scale=0.77]{gr-fib.pdf}
\end{VerbatimOut}

\MyIO

